Classification of obscuration-free reflective polygonal light beams

In this paper, we study the connected components of an obscuration-free planar polygonal light beam space modeling light propagation in optical systems composed of reflective surfaces and a focal plane. Through homotopy construction, we demonstrate that the connected components of this space are in bijection with the connected components of the reflective polygonal chains space, whose elements are the polygonal chains with their respective mirrors' orientations taken into account. In order to prove this, we introduce a topological invariant that provides an intelligible way for opticians to name homotopy-equivalent obscuration-free optical configurations thanks to previous work with polygonal chains.

==> figures/poly_chain.tex <==
This section presents the polygonal chains model derived in \cite{offaxis24}, which is the cornerstone of the beam light classification presented in the next sections.   
Here, we give the sketched ideas and refer the reader to \cite{offaxis24} for more details. 

Let us consider \(N+2\) points \((c_i)_{i = 0, \dots, N+1}\) in \(\mathbb{R}^2\)  to model the system: the half-line \((c_0, c_1]\) represents the direction of the source, the points \((c_j)_{j=1, \dots, N}\) correspond to the mirors, and \(c_{N+1}\) represents the focal plane.  
Thus, we work within the space of \(N\)-polygonal chains \(\LB\), defined by:
\[
\LB:= \bigl(\mathbb{R}^2 \bigr)^{N+2}
\]
with the topology induced by \(\bigl(\mathbb{R}^2 \bigr)^{N+2}\).  
Let us first introduce the notion of a ray for a polygonal chain.

\begin{definition}[Ray for a polygonal chain] \label{def:rayon ligne brisée}
Let \(L\) be an \(N\)-polygonal chain given by \((c_i) \in \LB\). We denote the \(j\)-th ray as  
\[
R_j = 
\begin{cases}
    (c_0, c_1] & \text{if } j = 0, \\
    [c_j, c_{j+1}] & \text{if } j \in \llbracket 1, N \rrbracket
\end{cases}
\]
for \(j \in \llbracket 0, N \rrbracket\).
\end{definition}

On $\LB$, $R_0$ can be empty if $c_0=c_1$ and $R_j$ for $j\in \llbracket 1, N \rrbracket$ can be reduced to a point if $c_j=c_{j+1}$. Hence, we are going to add constraints so that these degenerate cases are not in the admissible set and such that there is not obscurating or grazing rays so that there is no loss of information.
To achieve this, we will define the required polynomials and explain their geometric significance, in order to define a space for admissible polygonal chains.


\begin{definition}[\cite{offaxis24}]
    Let us define
\[
\begin{cases} 
P = X_1Y_2 - X_1Y_3 + X_2Y_3-X_2Y_1 + X_3Y_1 - X_3Y_2 \\
R = (X_2 - X_1)(X_3-X_1) + (Y_2 - Y_1)(Y_3-Y_1)
\end{cases}
\]

where $ P, Q\in \mathbb{R}[X_1,X_2,X_3,Y_1,Y_2,Y_3]$.
Let  \[P_{(i,j,k)}, \, R_{(i,j,k)} \in \mathbb{Q}[X_0, \dots, X_{N+1}, Y_0, \dots, Y_{N+1}] \text{ defined by}\] 
\begin{align*}
     P_{(i,j,k)} &= P(X_i, X_j, X_k, Y_i, Y_j, Y_k) \textrm{ for } 
    0\leq i<j<k \leq N+1\land \min(j-i, k-j) = 1\\
    R_{(i, j, k)} &= R(X_i, X_j, X_k, Y_i, Y_j, Y_k)\text{ for }  0 \leq i,j,k \leq N+1 \text{ distinct and }|i-j| = 1
\end{align*}
     


\end{definition} 
\noindent
The defined polynomials have a geometric significance when specializing  
\[
(X_0, \dots, X_{N+1}, Y_0, \dots, Y_{N+1}) \text{ to } (x_0, \dots, x_{N+1}, y_0, \dots, y_{N+1}) 
\]
where \(c_j = (x_j, y_j)\).  In particular: 

\begin{itemize}
    \item[(i)]The polynomial \(P_{(i,j,k)}\) equals 0 if and only if the points \(c_i\), \(c_j\), and \(c_k\) are collinear.  
    \item[(ii)]The polynomial \(R_{(i,j,k)}\) is greater than or equal to 0 when \(P_{(i,j,k)} = 0\) if and only if \(c_k \in [c_i, c_j)\). Indeed, with the specialization, we can write \(R_{(i,j,k)} = (c_j - c_i) \cdot (c_k - c_i)\).
\end{itemize}


We introduce below the space studied for Off-Axis classification presented in \cite{offaxis24}. To this end, we define the obscuration clause $\varphi_{(i,j,k)}$ associated with the index $(i,j,k)$, which is satisfied if and only if $c_k$ is within the segment $[c_i, c_j]$ for $(i,j,k) \in \widetilde{S}_{\obsc}$, where  
\[
\widetilde{S}_{\obsc} = \Bigl\{ (i, i+1, k), \, 1 \leq i \leq N , \, 1 \leq k \leq N+1, \, k \not \in \{ i, i+1\} \Bigr\}.
\]  
Using the observation made above regarding the polynomials $P_{(i,j,k)}$ and $R_{(i,j,k)}$, we have  
\[
\varphi_{(i,j,k)} = (P_{\sigma(i,j,k)} = 0) 
\wedge (R_{(k,i,j)} \leq 0),
%\wedge (R_{(i,j,k)} \geq 0) \wedge (R_{(j,i,k)} \geq 0),
\]  
for $(i,j,k) \in \widetilde{S}_{\obsc}$, and with $\sigma$ being the permutation that orders $i$, $j$, and $k$ from smallest to largest.  
Furthermore, in the case where $i=0$, the obscuration clause is satisfied if and only if $c_k$ lies in the half-line $(c_0, c_1]$ for $k \in \llbracket 2; N+1\rrbracket$. We then introduce the set of indices $\widetilde{S}_{\obsc}'$ defined as  
\[
\widetilde{S}_{\obsc}' = \bigl\{ (0,1,k), \, k = \llbracket 2, N+1\rrbracket\bigr\}.
\]  
The obscuration clause for  $(i,j,k)\in \widetilde{S}_{\obsc}'$ is given by  
\[
\varphi_{(i,j,k)} = (P_{(i,j,k)} = 0) \wedge (R_{(j,i,k)} \geq 0).
\]
It is easily seen that $\widetilde{S}_{\obsc} \cap \widetilde{S}_{\obsc}' = \varnothing$ showing that the $\varphi_{i,j,k}$ are well defined.


\begin{definition}[Obscuration] \label{def:obscuration}
We define the obscuration clause $\obsc$ as 
\[
\obsc:= \bigvee\limits_{(i,j,k) \in S_{\obsc}} \varphi_{(i,j,k)}
\]
where $S_{\obsc}:= \widetilde{S}_{\obsc} \cup \widetilde{S}_{\obsc}'$.
\end{definition}

\begin{figure}[h!]
  \begin{subfigure}[b]{.32\textwidth}
    \centering
      \includegraphics[width=\textwidth]{figures/ligne_brisee_cas1.pdf}
      \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
       \includegraphics[width=\textwidth]{figures/ligne_brisee_cas2.pdf}
      \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
       \includegraphics[width=\textwidth]{figures/ligne_brisee_rasante.pdf}
      \caption{}
  \end{subfigure}
  \caption{Non admissible polygonal chains: (a) the mirror $c_4$ is obscuring the ray $R_1=[c_1,c_2]$, (b) the mirror $c_4$ is obscuring the light source $R_0=(c_0,c_1]$ and (c) the mirror $c_2$ is grazing since it belongs to $[c_1,c_3]$.}
  \label{fig:obscuration_grazing}
\end{figure}

In Figure \ref{fig:obscuration_grazing}, we depict two broken $4$-lines that are obscured. The one shown in (a) satisfies $\varphi_{(1,2,4)}$ because $c_4$ belongs to the segment $[c_1, c_2]$. The second (depicted in (b)) is obscured because we observe that $c_4$ lies on the light source: $c_4$ belongs to $(c_0, c_1]$. Thus, $\varphi_{(0,1,4)}$ is satisfied for the polygonal chain $c = (c_0, \dots, c_5)$, and therefore, the polygonal chain is obscured.

\begin{remark} \label{rem:obscuration}
    The obscuration clause $\obsc$ for the polygonal chain $L = (c_i) \in \LB$ can be equivalently rewritten using the concept of a ray:  
\[
\obsc = \bigvee_{0 \leq j \leq N} \bigvee_{\substack{1 \leq k \leq N+1 \\ k \neq j,j+1}} \bigl( R_j \cap c_k \neq \varnothing \bigr).
\]
\end{remark}


\bigskip

We now introduce a new clause defining grazing, i.e., the cases where the polygonal chain has three consecutive points aligned in order.  
To this end, we introduce the set \( S_{\ras} = \{ (m-1,m,m+1) \, , \, 1 \leq m \leq N \} \) and define the grazing clause for indices \((i,j,k)\) in \(S_{\ras}\):  
\[
\psi_{(i,j,k)} = \bigl( P_{(i,j,k)} = 0 \wedge R_{(j,i,k)} \leq 0 \bigr).
\]

\begin{definition}[Grazing] \label{def:rasance}
We define the grazing clause $\ras$ as 
\[
\ras:= \bigvee\limits_{(i,j,k) \in S_{\ras}} \psi_{(i,j,k)}.
\]
\end{definition}
\begin{remark}\label{re:grazing}
    The grazing clause $\ras$ holds true if a degenerate ray exists. Indeed, if $R_0=\emptyset$ then $\psi_{(0,1,2)}=\texttt{true}$ and if there exists $j\in \llbracket 2,N\rrbracket$ such that $R_j=\{c_j\}$ then $\psi_{j-1,j,j+1}=\texttt{true}$.
\end{remark}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.6\textwidth]{figures/ligne_brisee_rasante.pdf}
%     \caption{Grazing polygonal chain.}
%     \label{fig:rasance}
% \end{figure} 

In \Cref{fig:obscuration_grazing}-(c), the points $c_1$, $c_2$, and $c_3$ are aligned, so $P_{(1,2,3)}(c) = 0$ and $R_{(2,1,3)} < 0$, where $c$ is the polygonal chain represented in the figure. Thus, the grazing clause $\psi_{(1,2,3)}$ is satisfied for this polygonal chain so that the system is grazing.


\begin{definition}[Space $\LO$] \label{def:LO}
We first define the joint clause of obscuration and grazing as $\ObscRas = \obsc \vee \ras$. The non-admissible polygonal chains subspace is defined as \( E_{\ObscRas} = \bigl\{ c \in \LB\,: \, \ObscRas(c) \bigr\} \). We then define the space of $N$-polygonal chains under obscuration and grazing constraints as:  
\[
\LO:= \LB \backslash E_{\ObscRas}.
\]
\end{definition}

\begin{definition} [Exact Invariant: Off-Axis Nomenclature] \label{def nomenclature}  
We introduce the nomenclature, denoted as  
\begin{align*}  
\N: \LO \rightarrow \pi_0 \bigl(\LO \bigr),  
\end{align*}  
where $\pi_0(\LO)$ is the set of connected components of $\LO$. We define $\N$ by taking $\N(L) = \N(L')$ if and only if $L$ and $L'$ are in the same connected component of $\LO$, for $L$ and $L'$ in $\LO$.  
\end{definition}



The nomenclature is therefore by definition an exact invariant in the sense of \cref{def:invariant}: it is even the canonical exact invariant since it directly uses the connected components of the space.


\bigskip

We have an explicit characterization of the nomenclature called the GOFFA nomenclature. This nomenclature, denoted by $\NGOFFA$, is introduced in \cite{offaxis24}, and the following theorem shows that it is an exact invariant in specific cases.


\begin{theorem}[\cite{offaxis24}] \label{théorème_nomenclature}
    The nomenclature given by $\NGOFFA: \LO \rightarrow B$ is an invariant of the space $\LO$. It is an exact invariant for $N= 3,4$ mirrors.
\end{theorem}


Let us explain in more detail how the nomenclature $\NGOFFA$ assigns a name to each polygonal chain. The name of a system is given recursively on its mirrors. For a polygonal chain $L = (c_i)_{0 \leq i \leq N+1} \in \LO$, we process the mirrors step by step in the order $j = 1, \dots, N$.

At step $j$, we consider the segment $[c_j, c_{j+1}]$. If this segment does not intersect any of the previous segments $[c_k, c_{k+1}]$ for $1 \leq k < j$ or the light source $(c_0, c_1]$, then we assign the letter $V$ to the $j$-th mirror. Otherwise, we assign the letter $X$, and we also indicate as subscripts the segments and/or the half-line (for the light source) that are intersected by the segment $[c_j, c_{j+1}]$. 

Furthermore, we add the letter $A$ or $C$ ($A$ for \emph{anticlockwise} and $C$ for \emph{clockwise}) as a subscript to indicate the direction of rotation of the ray at the $j$-th mirror. This is explicitly given by the sign of $(c_{j+1}-c_j) \wedge (c_{j-1}- c_j)$, where $\wedge$ is the cross product given by  
\[
\begin{pmatrix}x \\ y \end{pmatrix} \wedge \begin{pmatrix}x' \\ y' \end{pmatrix} = xy' - x'y'.
\]
For $N=3$, these 3 invariants are sufficient. For $N=4$, an additional invariant that considers the set of points enclosed by a subset of the polygonal chain is necessary.
Thus, we observe that, up to symmetry with respect to the first mirror, all names begin with $V_A$.  
The space $\text{LO}^3(\mathbb{R}^2)$ has 32 connected components and 16 up to symmetry while the space $\text{LO}^4(\mathbb{R}^2)$ has 288 connected components and 144 up to symmetry.


==> inputs/beam.tex <==
In order to introduce the space $\Faisc$ of obscuration-free and non-grazing beams, we start by introducing the space of primary beams.
% We define a topological invariant $\IFaisc$ for this space that comes from the characteristic $\Car$ for $\LR$ (see definition \ref{def:caracteristique}) and from the nomenclature $\N$ for $\LO$ (see definition \ref{def nomenclature}). Finally, we show that $\IFaisc$ is an exact invariant with theorem \ref{thm invariance}.

\begin{defi}[Primary beam]
    Let $N \in \mathbb{N}^*$, an $N$-primary beam is the data 
    \[
    \Bigl((a_i)_{0 \leq i \leq N+1}, (b_i)_{0 \leq i \leq N+1}\Bigr)\in \LB\times \LB
    \]
    of two polygonal chains of $\mathbb{R}^2$ verifying the following assumptions:
    \begin{itemize}
        \item[$\circ$] for $1 \leq k \leq N$, $a_k \neq b_k$,
        \item[$\circ$]  $a_0 = b_0=(-1,0)$ and $a_{N+1}=b_{N+1}$,
        \item[$\circ$] $ c_1=\frac{a_1 + b_1}{2}=(0,0)$.
    \end{itemize}
\end{defi}

In this definition, we exclude degenerate beams to ensure that the line $(a_0 c_1]$, representing the direction of the light source, is well-defined, and equal (without loss of generality)   to the half-axis of negative $y$-values and that the mirrors $[a_kb_k]$ have a strictly positive length. The condition $a_{N+1}=b_{N+1}$ means that the beam is convergent at the focal plane.

We denote the space of $N$-primary beams $\FaiscP$. The topology we consider is the classical topolology induced by $\bigl(\mathbb{R}^2 \bigr)^{2(N+2)}$ on $\FaiscP$. 

\begin{defi}[The $t$-polygonal chain of a primary beam $F$] \label{def:t-ligne brisee}
Let $F$ be an $N$-primary beam  given by $(a_i)$ and $(b_i)$. 
Let $t \in[0,1]$, let us define $s_t$ that depicts the direction of the source for the $t$-polygonal chain of $F$ with $s_t = (1-t)a_1 + tb_1 + a_0$. \\
The $t$-polygonal chain $P_t$ is then defined recursively as the $N$-polygonal chain $P_t = (P_i^t)_{0 \leq i \leq N+1}$ with: 
\[
P_i^t = \begin{cases}
    s_t \text{ if } i = 0, \\
    (1-t)a_1 + tb_1 \text{ if } i = 1, \\
    \left.
    \begin{aligned}
    &(P_{i-1}^t, I_{i-1}^i) \cap [a_i,b_i] \text{ if } 
    (a_{i-1}, a_i) \cap (b_{i-1}, b_i) \neq \varnothing, \\
    &(1-\lambda_{i-1})a_i + \lambda_{i-1}b_i \text{ otherwise}.
    \end{aligned} \right\rbrace\text{ if }i\in\llbracket2,N+1\rrbracket
\end{cases}
\]
where $I_{i-1}^i = (a_{i-1}, a_i) \, \cap \, (b_{i-1}, b_i )$ when $(a_{i-1}, a_i) \, \cap \, (b_{i-1}, b_i) \neq \varnothing$ and $\lambda_k$ ($1 \leq k \leq N$) is the real number between $[0,1]$ such that $P_k^t = (1-\lambda_k)a_k + \lambda_k b_k $. \\
We say that $P_i^t$ is the $i$-th impact point of the $t$-polygonal chain.
\end{defi}

Let us notice that the extremal $t$-polygonal chains of $F$ are the polygonal chains $(a_i)$ and $(b_i)$, that is to say
\[
P_0 = (a_i)_{0 \leq i \leq N+1}  \quad \text{ and } \quad P_1 = (b_i)_{0 \leq i \leq N+1}.
\]
Thanks to  \cref{def:t-ligne brisee}, we have a parametrization of $t$-polygonal chains 
\begin{align*}
    P: [0,1] & \longrightarrow L^N(\mathbb{R}^2) \\
    t & \longmapsto P_t
\end{align*}
that connects the two polygonal chains $(a_i)$ and $(b_i)$. \\

\begin{defi}[Ray of a $t$-polygonal chain]  \label{def:rayon t-ligne brisee}
Let us consider the $t$-polygonal chain $P_t$ of the primary beam $F$ (see  \cref{def:t-ligne brisee}). We define for $j$ in $\llbracket 0, N \rrbracket$, the $j$-th ray $R_j^t$ of the $t$-polygonal chain as in  \cref{def:rayon ligne brisee}:  
\[
R_j^t = \begin{cases}
(P_0^t, P_1^t]  \text{ if } j=0, \\
[P_j^t, P_{j+1}^t] \text{ if }j\in \llbracket 1,N\rrbracket.
\end{cases}
\]
\end{defi}


\begin{defi}[Centered polygonal chain] \label{def:ligne brisee centrale}
Let $F$ be an $N$-primary beam given by the polygonal chains $(a_i)$ and $(b_i)$. We define the application $M$ as 
\begin{align*}
    M: \FaiscP &\longrightarrow \LB \\
    F &\longmapsto P_\frac{1}{2} = \Bigl( P_j^{\frac{1}{2}} \Bigr)_{0 \leq j \leq N+1}.
\end{align*}
We say that $M(F)$ is the centered polygonal chain of $F$.
\end{defi}

\begin{defi}[Beam] \label{def:faisceau}
    Let $N \in \mathbb{N}^*$, an $N$-beam $F$ is an $N$-primary beam given by $(a_i)$ and $(b_i)$ verifying the following assumptions: 
    \begin{itemize}
        \item[$\circ$] (Non-obscuration) \label{condition non-obscuration} \\
        we have for all $0 \leq j \leq N$, $1 \leq k \neq j,j+1 \leq N+ 1$ and $t$ in $[0,1]$
        \[
        R_j^t \cap S_k = \varnothing
        \]
        
        where $S_k = [a_kb_k]$ is the $k$-th mirror,
        \item[$\circ$] (reflection) \label{condition reflection} \\
        We have for all $1 \leq i \leq N$ 
        \begin{multline*}
        \sgn \bigl((a_{i-1}-a_{i})\cdot n_i \bigr) = \sgn \bigl((b_{i-1}-b_{i})\cdot n_i \bigr) = \\\sgn \bigl((a_{i+1}-a_{i})\cdot n_i \bigr) =\sgn \bigl((b_{i+1}-b_{i})\cdot n_i \bigr) \neq 0
        \end{multline*}
        where $n_i$ is the unit normal vector of $i$-th mirror $[a_ib_i]$ and $\sgn$ the sign function.
        % given by:
        % \begin{align*}
        %     \sgn: \mathbb{R} & \longrightarrow \{ -1, 0, 1 \} \\
        %     x & \longmapsto \begin{cases}
        %         1 \text{ if } x>0, \\
        %         -1  \text{ if }  x<0, \\
        %         0 \text{ if } x=0.
        %     \end{cases}
        % \end{align*}
    \end{itemize}
\end{defi}

We denote $\Faisc$ the space of $N$-beams. The topology we consider is the topology induced by $\bigl(\mathbb{R}^2\bigr)^{2(N+2)}$. 
In  \Cref{fig:faisceau_intro}-(a),  \cref{def:faisceau} is depicted with the example of a $3$-beam. Let us notice that this beam respects the conditions of non-obscuration and reflection which define a beam.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.6\textwidth]{figures/faisceau_non_obscure.pdf}
%     \caption{A beam $F$ composed of three mirrors}
%     \label{fig:faisceau}
% \end{figure}   

\begin{remark} [Reflection] \label{remarque reflection}
    The reflection condition of a beam is equivalent to tell that the points $a_{i-1}$, $b_{i-1} $, $a_{i+1} $ and  $b_{i+1} $ are in the same half-plane of boundary $(a_i b_i)$. Then, the convex hull $\text{\normalfont{Conv}}(a_{i-1}, b_{i-1}, a_{i+1}, b_{i+1})$ is in the same half-plane of boundary $(a_ib_i)$.
\end{remark}
\begin{remark}\label{remarque semi-algebraic}
    We can show that the space of beams $\Faisc$ is a semi-algebraic set\footnote{\label{footnote:sas} Semi-algebraic sets in $\mathbb{R}^n$ are subsets of $\mathbb{R}^n$ formed by Boolean combinations of sets of the form ${ (x_1, \dots, x_n) \in \mathbb{R}^n , | , P(x_1, \dots, x_n) \geq 0 }$ for $P \in \mathbb{R}[X_1, \dots, X_n]$. By Boolean combinations, we refer to finite combinations of unions, intersections, and complements.} since the geometric conditions of non-obscuration and reflection can be expressed using only Euclidian geometry conditions which can be translated into polynomial inequalities.
\end{remark}

\begin{lemme}[Property of $t$-polygonal chains of $F$] \label{lemme:t-ligne brisee}
    Let $F \in \Faisc$, every $t$-polygonal chain $P_t$ of $F$ (according to definition \ref{def:t-ligne brisee}) belongs to $\LO$ for $t$ in $[0,1]$.
\end{lemme}

\begin{proof}
    We will show the contraposition and we consider then that $P_t$ (for $t$ in $[0,1]$) is a polygonal chain verifying $\ObscRas$. We then have two possibilities:
    \begin{itemize}
        \item[$\circ$] $L$ verifies $\obsc$. There exists $0 \leq j \leq N$ and $1 \leq k \neq j, j+1 \leq N+1$ such that $P_j^t \cap c_k \neq \varnothing$ by  \cref{rem:obscuration}. Thus, we have $R_j^t \cap S_k \neq \varnothing$ as $c_k \in S_k$. Hence, the non-obscuration condition is not verified and $F$ is not a beam then.
        \item[$\circ$] $L$ verifies $\ras$. There exists $1 \leq i \leq N$ such that $P_i^t$ belongs to $[P_{i-1}^t,P_{i+1}^t]$. Therefore, we have $[P_{i-1}^t,P_{i+1}] \cap (a_i b_i) \neq \varnothing$ as $P_i^t$ belongs to $[a_i,b_i]$. Thus, $\text{Conv}(a_{i-1},b_{i-1},a_{i+1},b_{i+1})$ is not in the same half-plane of boundary $(a_i b_i)$, the reflection condition is then not verified (\cref{remarque reflection}).
    \end{itemize}
\end{proof}

\begin{remark} \label{rem:ligne brisees centrale faisceau}
    With  \cref{lemme:t-ligne brisee}, the application $M$ defined in \cref{def:ligne brisee centrale} induces an application $\widetilde{M}: \Faisc \rightarrow \LO$ where $\widetilde{M} = M|_{\Faisc}$. We denote this application $M$ in the sequel by abuse of notation. 
\end{remark}

\begin{defprop}[Application $M_R$]
    An $N$-beam $F$ given by $(a_i)$ et $(b_i)$ induces a reflexive polygonal chain through the application:
    \begin{align*}
        M_R: \Faisc & \xlongrightarrow{(M,A)} \LR \\
        F & \longmapsto \Bigl(M(F), \bigl(A(a_j-b_j)\bigr)_{1 \leq j \leq N} \Bigr)
    \end{align*}
    where $M: \Faisc \rightarrow \LO$ is given by  \cref{rem:ligne brisees centrale faisceau} and $A: \mathbb{R}^2 \rightarrow \mathbb{R}/2 \pi \mathbb{Z}$ is the angle function that returns the angle $\theta$ to $x \neq 0$ such that $x = r \bigl(\cos( \theta), \sin(\theta) \bigr)$ for a unique $r > 0$.
\end{defprop}
    
\begin{proof}
    We have that $M(F)$ belongs to $\LO$ by  \cref{lemme:t-ligne brisee}. Moreover, as the beam $F$ verifies the reflection condition of beams, we have that $a_{j-1}$, $b_{j-1} $, $a_{j+1} $ and $b_{j+1} $ are in the same half-plane of boundary $(a_j b_j)$, by  \cref{remarque reflection}, for $j$ in $\llbracket 1, N \rrbracket$. This implies that points $c_{j-1}$ and $c_{j+1} $ are in the same half-plane with the boundary  line passing through $c_j$ of angle $\theta_j$ where we consider $(c_i)_{0 \leq i \leq N+1}:= M(F)$ and $\theta_j:= A(a_j - b_j) $.
\end{proof}

\begin{defi} [Beam homotopy]
Let us consider two $N$-beams $F$ et $F'$ given respectively by $\bigl((a_i),(b_i)\bigr)$ and $\bigl((a_i'),(b_i')\bigr)$, we say that $F$ and $F'$ are \textit{homotopic} if there exists an application 
\[
H: \bigl( \llbracket 0, N+1 \rrbracket \sqcup \llbracket 0, N+1 \rrbracket \bigr) \times [0,1] \longrightarrow \mathbb{R}^2
\]
such that $\begin{cases}
H(\cdot, 0) = F \text{, that is to say } H(p_1(i), 0) = a_i \text{ et } H(p_2(i), 0) = b_i \\
H(\cdot, 1) = F' \\
H(\cdot, t) \in \Faisc \text{ for all } t \text{ in } [0,1]
\end{cases}$ \\
where $p_1, p_2: \llbracket 0, N+1 \rrbracket \longmapsto \llbracket 0, N+1 \rrbracket \, \sqcup \, \llbracket 0, N+1 \rrbracket$ are the two canonical applications of the union. 
We note $F \cong F'$ to mean that $F$ and $F'$ are homotopic.
\end{defi}

Let us notice that $F \cong F'$ is equivalent to the existence of a continuous path $\gamma: [0,1] \rightarrow \Faisc$ such that $\gamma(0) = F$ and $\gamma(1) = F'$.

\medskip

Before giving the next proposition, we recall that a polygonal chain $(z_i)_{0 \leq i \leq N+1}$ in $\LO$ has a nomenclature $\N \bigl((z_i)\bigr)$ which returns the connected component of $\LO$ in which $(z_i)$ belongs (see  \cref{def nomenclature} for more details).

\begin{prop} \label{nomenclature faisceau}
Let $F$ be an $N$-beam given by $(a_i)$ et $(b_i)$, then $\N \bigl((a_i)\bigr) = \N \bigl((b_i)\bigr)$, that is $(a_i)$ et $(b_i)$ are in the same connected component of $\LO$. \\
More generally, we have for $t, t'$ in $[0,1]$, $\N(P_t) = \N(P_{t'})$. 
\end{prop}

\begin{proof}
    We use the parametrization of rays 
    \begin{align*}
        P: [0,1] & \longrightarrow \text{L}^N(\mathbb{R}^2) \\
        t & \longmapsto P_t
    \end{align*}
    by  \cref{lemme:t-ligne brisee} which tells us that every $t$-ray of $F$ is obscuration-free that is: $ \forall \, t \in [0,1], \, P_t\in\LO$. By denoting $P:[0,1]\ni t\mapsto P_t\in \LB$, we get the induced application $\widetilde{P}$ (indicated by the dashed arrow) in the following commutative diagram: 
    \begin{center}
        \begin{tikzcd}
    & \LO \arrow[hookrightarrow]{d} \\
    {[0,1]} \arrow{r}{P} \arrow[dashed]{ur}{\widetilde{P}} & \text{L}^N(\mathbb{R}^2)
    \end{tikzcd}
    \end{center}
    Moreover, we have $\widetilde{P}(0) = (a_i)$ and $\widetilde{P}(1) = (b_i)$. So $\widetilde{P}$ is a path in $\LO$ connecting  $(a_i)$ and $(b_i)$, they are then in the same connected component and we obtain $\N\bigl((a_i)\bigr) = \N\bigl((b_i)\bigr)$. \\
    We also use the application $\widetilde{P}$ to show that $\N(P_t) = \N(P_{t'})$ with $t,t' \in [0,1]$ by remarking that $\widetilde{P}(t) = P_t$ and $\widetilde{P}(t') = P_{t'}$; we then have a path between $P_t$ and $P_{t'}$ in $\LO$.
\end{proof}

\begin{defi}[$\NFaisc$ nomenclature]
    We define the nomenclature $\NFaisc$ in the beams space $\Faisc$ as
    \begin{align*}
        \NFaisc: \Faisc &\longrightarrow \pi_0(\LO) \\
        F &\longmapsto \N (M(F))
    \end{align*}
    where $M$ is the application defined in  \cref{rem:ligne brisees centrale faisceau}.
\end{defi}

 \Cref{nomenclature faisceau} tells us that the nomenclature of a beam does not depend on the chosen ray: we could as well take $\N \bigl((a_i)\bigr)$ or $\N \bigl((b_i)\bigr)$ instead of $\N \bigl(M(F)\bigr)$ since these nomenclatures are all the same. Thus, the $\NFaisc$ nomenclature is a well-defined notion for a beam.

\begin{defi}[Characteristic of a beam: $\CarFaisc$]
    Let $F$ be an $N$-beam. The \textit{characteristic} of the beam $F$ is defined by extension as  
    \[
    \CarFaisc(F):= \Car(M_R(F)).
    \]
\end{defi}

% For all $j$ in $\llbracket 1, N \rrbracket$, we say that the $j$-th subbeam of an $N$-beam $F$ is \emph{direct} if and only if $\CarFaisc(F)_j = 1$.


In \Cref{fig:faisceau invariant}, we represent in the upper half the beam we had shown in \Cref{fig:faisceau_intro}-(a) with the centered polygonal chain $M(F)$ added in blue in the figure. In the lower half, we then consider $M(F)$ only and we give the nomenclature of the beam  and we represent the angles $\theta_j$ of $M_R(F)$ with arrows (in orange when $\theta_j \in \Aplus$ and in green when $\theta_j \in \Aminus$).

\begin{figure}[h!]
    \centering
    \label{fig:a}
    \begin{subfigure}{0.45\textwidth}
         \includegraphics[width=\textwidth]{figures/faisceau_et_rayon_central.pdf}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
         \includegraphics[width=\textwidth]{figures/caracteristique_nomenclature.pdf}
    \end{subfigure}
    \caption{A beam $F$, its nomenclature and characteristic}
    \label{fig:faisceau invariant}
\end{figure}   


\medskip

So far, we have introduced the $\NFaisc$ nomenclature and $\CarFaisc$ characteristic. We use in the rest the conjunction $\IFaisc$ of these two application to obtain an invariant of $\Faisc$.

\begin{prop}[Topological invariant: $\IFaisc$] \label{prop:invariance}
    Let $F$ and $F'$ be two beams in $\Faisc$ such that $F \cong F'$, then
    \[
    \IFaisc(F) = \IFaisc(F')
    \]
    where we define the application $\IFaisc$ as 
    \begin{align*}
        \IFaisc:= \bigl( \NFaisc \times \CarFaisc \bigr): \Faisc &\longrightarrow \pi_0(\LO) \times \{ -1, 1\}^N \\
        F &\longmapsto \bigl(\NFaisc(F), \CarFaisc(F)\bigr).
    \end{align*}
\end{prop}

\begin{proof}
    Let us consider $F$ and $F'$ such that $F \cong F'$, then, there exists  a path $\gammaFaisc$ in $\Faisc$ between $F$ and $F'$. Consider now the function $M_R \circ \gammaFaisc: [0,1] \rightarrow \LR $ that connects $L:= M_R(F)$ to $L':= M_R(F')$, we have 
    \[
    \IR(L) = \IR(L')
    \]
    since $\IR:= \bigl( \NR \times \Car \bigr)$ is a topological invariant by  \cref{corollaire:LR invariant}. This means that we have
    \begin{gather*}
        \NR(L) = \NR(L'), \quad 
        \Car(L) = \Car(L'),
    \end{gather*}
    and we then find
    \begin{gather*}
        \NFaisc(F) = \NR(L) = \NR(L') = \NFaisc(F'), \\
        \CarFaisc(F) = \Car(L) = \Car(L') = \CarFaisc(F').
    \end{gather*}
    Thus, we obtain 
    \[
    \IFaisc(F) = \bigl( \NFaisc(F), \CarFaisc(F) \bigr) = \bigl( \NFaisc(F'), \CarFaisc(F') \bigr) = \IFaisc(F'),
    \]
    what shows the proposition.
\end{proof}

 In the following part, we introduce definitions and results that we use in order to show  \cref{thm invariance} which shows that $\IFaisc$ is an exact invariant.

\begin{defi}[$P_l$ application] \label{def application P_l}
We define the $P_l$ application with parameter\\ $l:= \bigl( (l_j^a)_{1 \leq j \leq N}, (l_j^b)_{1 \leq j \leq N} \bigr) \in \bigl((\mathbb{R}^+_*)^N\bigr)^2$ as 
\begin{align*}
    P_l: \LR &\longrightarrow \FaiscP \\
    \bigl((c_i), (\theta_j)\bigr) &\longmapsto \bigl((a_i),(b_i)\bigr)
\end{align*}
with 
\[
(a_i, b_i) = \begin{cases}
    (c_i,c_i) \text{ if } i \in \{0, N+1\} \\
    \Bigl( c_i + l_i^a \bigl(\cos(\theta_i),\sin(\theta_i)\bigr), c_i - l_i^b \bigl( \cos(\theta_i),\sin(\theta_i) \bigr) \Bigr) \text{ if } i \in \llbracket 1, N \rrbracket
\end{cases}
\]
\end{defi}

\begin{defi}[$d_R$ function]
    We introduce the continuous function $d_R$ representing the minimal mirror-to-mirror distance for a reflexive polygonal chain
    \begin{align*}
        d_R: \LR &\longrightarrow \mathbb{R}^+_* \\
        \bigl((c_i), (\theta_j)\bigr) &\longmapsto \min\limits_{1 \leq i \leq N} \min \Bigl(\bigl|(c_{i-1}- c_i) \cdot n(\theta_i)\bigr|, \bigl|(c_{i+1} - c_i) \cdot n(\theta_i)\bigr| \Bigr) 
    \end{align*}
    where $n$ is the function that gives the unit normal vector to an angle.
\end{defi}

The terms $|(c_{i-1}-c_i) \cdot n(\theta_i)|$ that we use in order to define the application, represents the distance between the point $c_{i-1}$ and the line $d(\theta_i)$ of direction $\theta_i$ and crossing $c_i$. In the same manner, $|(c_{i+1}-c_i) \cdot n(\theta_i)|$ is the distance between the point $c_{i+1}$ and the line $d(\theta_i)$.

\begin{prop} \label{prop faisceau P_l condition reflection}
    Let $L$ be an $N$-reflexive polygonal chain given by $\bigl((c_i), (\theta_j)\bigr)$ and $P_l(L)$ the primary beam given by $\bigl((a_i),(b_i)\bigr)$  as stated in \cref{def application P_l}. Assume 
    \[
    K:= \max\limits_{1 \leq j \leq N} \max(l_j^a, l_j^b)  < d_R(L),
    \]
    then the reflection condition of a beam (stated in \cref{condition reflection}) is verified by $F$.
\end{prop}

\begin{proof}
First of all, we have by definition of $d_R$
\begin{gather*}
    d \bigl( c_{i-1}, (a_i b_i) \bigr) \geq d_R(L) \; \text{ and } \; d \bigl( c_{i+1}, (a_i b_i) \bigr) \geq d_R(L)
\end{gather*}
for all $i$ in $\llbracket 1, N \rrbracket$, where for $x \in \mathbb{R}^2$ and $Y \subseteq \mathbb{R}^2$, we define $d(x, Y)$ as 
\[
d(x, Y):= \inf\limits_{y \in Y} |x-y|
\]
We indeed observe that 
\begin{align*}
    d \bigl( c_{i-1}, (a_i b_i) \bigr) &= |(c_{i-1} - c_i) \cdot n(\theta_i)|, \\
    d \bigl( c_{i+1}, (a_i b_i) \bigr) &= |(c_{i+1} - c_i) \cdot n(\theta_i)|.
\end{align*}

By  \cref{remarque reflection}, the reflection condition returns to verifying for some $N$-beam given by $\bigl( (x_i),(y_i) \bigr)$ if the points $x_{i-1}$, $y_{i-1}$, $x_{i+1}$, $y_{i+1}$ are in the same half-plane of boundary $(x_i y_i)$ for $i$ in $\llbracket 1, N \rrbracket$. In our case, we have $c_{i-1}$ and $c_{i+1}$ in the same half-plane of boundary $d(\theta_i)$, the line produced by the angle $\theta_i$ as $L$ is in $\LR$. \\
If we then take
\[
K < d_R(L),
\]
we have $|a_{i-1} - c_{i-1}| = l_{i-1}^a < d_R(L)$ and $d\bigl(c_{i-1}, (a_i b_i) \bigr)  \geq d_R(L)$ for all $i$ in $\llbracket 1,N \rrbracket$ and so $a_{i-1}$ et $c_{i-1}$ are in the same half-plane of boundary $(a_i b_i)$. We can do the same reasoning with the couples of points $(b_{i-1}, c_{i-1} )$, $(a_{i+1}, c_{i+1})$ et $(b_{i+1}, c_{i+1})$ to show that they are in the same half-plane of boundary $(a_i b_i)$. \\
Thus, the points $a_{i-1}$, $b_{i-1}$, $a_{i+1}$ and $b_{i+1}$ are in the same half-plane of boundary $(a_i b_i)$ and the reflection condition is then verified.    
\end{proof}


\begin{defi}[$d_O$ function]
    We introduce the continuous function $d_O$ representing the distance of the rays to the mirrors (not adjacent) for a reflexive polygonal chain
    \begin{align*}
    d_O: \LR &\longrightarrow \mathbb{R}^+_* \\
    \bigl((c_i), (\theta_j)\bigr) &\longmapsto \min_{0 \leq j \leq N} \min_{\substack{1 \leq k \leq N+1 \\ k \neq j,j+1}} d(c_k,R_j)
    \end{align*}
    where $d(x,Y) = \inf\limits_{y \in Y} |x-y|$ with $x \in \mathbb{R}^2$ and $Y \subseteq \mathbb{R}^2$ and where $R_j$ is the $j$-th ray ray of the reflexive polygonal chain (see  \cref{def:rayon_LR}).
\end{defi}


    
\begin{lemme} \label{lemme faisceau P_l condition non obscuration}
    Let $L$ be an $N$-reflexive polygonal chain given by $\bigl((c_i), (\theta_j)\bigr)$ and $F:= P_l(L)$, with $l = \bigl( (l_j^a, l_j^b) \bigr)$, the primary beam given by $\bigl((a_i),(b_i)\bigr)$. We have the two following results: 
    \begin{enumerate}
        \item \(
        \forall \, k \in \llbracket 1,N+1 \rrbracket, \forall \, w \in S_k, |w-c_k| \leq \max(l_k^a, l_k^b)
        \) where $S_k = [a_kb_k]$,
        \item 
        \(\forall \, j \in \llbracket 0, N \rrbracket, \forall \, t \in [0,1], \forall \, z \in R_j^t \text{ ($t$-polygonal chain of $F$)} \)
        \[
        \exists \, x \in R_j \text{ ($j$-th ray of L)}, \text{ such that } |z-x| \leq K
        \]
        with $K:= \max\limits_{1 \leq j \leq N} \max (l_j^a, l_j^b)$.
        
    \end{enumerate}
\end{lemme}

\begin{proof}
Result 1. comes directly from the definition of $P_l$. \\ 
We show result 2. by considering the set 
\[
X_j = \bigcup\limits_{x \in R_j} B^f(x, K)
\]
with $j$ fixed and where $B^f(x, K)$ is the closed ball of center $x$ and of radius $K$.
We must show that all $z$ in $R_j^t$ belongs to $X_j$. \\
We can assume without loss of generality that $c_j = (0,0)$ and $c_{j+1} = (0,v)$ with $v > 0$ by using a translation and a rotation. The set $X_j$ can then be rewritten as 
\[
X_j = \begin{cases}
    B^f( c_{j+1}, K) \, \cup \, \bigl( [C,D] + \mathbb{R}^-_y \bigr) \text{ if } j=0 \\
    B^f( c_j, K) \, \cup \, ABCD \, \cup \, B^f( c_{j+1}, K) \text{ if } j \in \llbracket 1, N \rrbracket
\end{cases}
\]
where $ABCD$ is the rectangle given by the points $A = (-K, 0)$, $B = (K, 0)$, $C = (K, v)$, $D = (-K, v)$ and $\mathbb{R}^-_y = \{ (0, \tau) \,: \, \tau \in \mathbb{R}^- \}$. It is clear that the set  $X_j$ is convex from this description. We represent in  \Cref{fig:lemme P_l} the sets $X_j$ with $X_0$ in (a), and the other cases in (b). 
    
\begin{figure}[h!]
\centering
  \begin{subfigure}[b]{.35\textwidth}
    \centering
      \includegraphics[
angle=-90,width=\textwidth]{figures/X_0_rotate.pdf}
      \caption{The set $X_0$}
  \end{subfigure}
  \centering
  \begin{subfigure}[b]{0.35\textwidth}
    \centering
     \includegraphics[
angle=-90,width=\textwidth]{figures/X_j_rotate.pdf}
      \caption{The set $X_j$ for $j = 1, \dots, N$}
  \end{subfigure}
  \caption{}
  \label{fig:lemme P_l}
\end{figure}

Let us consider the convex hull $E_j:= \text{Conv}(a_j, b_j ,a_{j+1}, b_{j+1})$, we obtain $R_j^t$ included in $E_j$. Now, as $a_j, b_j, a_{j+1}, b_{j+1} $ belong to $X_j$ (by result 1.) and that $X_j$ is convex, we then have $E_j \subseteq X_j$ and $R_j^t \subseteq X_j$.
\end{proof}

\begin{prop} \label{prop faisceau P_l condition non obscuration}
    Let $L$ be an $N$-reflexive polygonal chain given by $\bigl((c_i), (\theta_j)\bigr)$ and $F:= P_l(L)$ with  $l = \bigl( (l_j^a, l_j^b) \bigr)$, the primary beam given by $\bigl((a_i),(b_i)\bigr)$. Assume \[
    K:= \max\limits_{1 \leq j \leq N} \max \bigl( l_j^a, l_j^b \bigr) < \frac{d_O(L)}{2},
    \]
    then the non-obscuration condition of a beam (stated in \cref{condition non-obscuration}) is verified by $F$. 
\end{prop}

\begin{proof}
    Let us take $w$ in $S_k = [a_k,b_k]$ and $z$ in $R_j^t$ with $0 \leq j \leq N$  and  $1 \leq k \leq N+1$ such that $k \neq j, j+1$. By lemma \ref{lemme faisceau P_l condition non obscuration}, we have 
    \begin{gather*}
        |w-c_k| \leq K \qquad
        |z-x| \leq K 
    \end{gather*}
    with $x$ in the $j$-th ray $R_j$ of $L$. \\
    Thus, we obtain
    \[
    |z-w| \geq |x-c_k| - |z-x| - |w-c_k| \geq d_O(L) - K - K
    \]
    since $|x-c_k| \geq d_O(L)$ by the definition of $d_O$. \\
    So we have 
    \[
    |z-w| \geq d_O(L) - 2K > 0.
    \]
    by the hypothesis $K < \frac{d_O(L)}{2}$ and then the non-obscuration condition
    \[
    S_k \cap R_j^t = \varnothing.
    \]
    is verified.
\end{proof}

\begin{corollaire} \label{corollaire faisceau P_l}
    Let $L$ be an $N$-reflexive polygonal chain and $F$ given by $P_l(L)$. Assume 
    \[
    K:= \max\limits_{1 \leq j \leq N} \max (l_j^a,l_j^b) < \min\Bigl(d_R(L), \frac{d_O(L)}{2} \Bigr),
    \] 
    then $F$ is a beam. 
\end{corollaire}

\begin{proof}
    By propositions \ref{prop faisceau P_l condition reflection} and \ref{prop faisceau P_l condition non obscuration}, we have that $F$ verifies the two necessary conditions to be a beam.
\end{proof}

\begin{prop}[Homotopy with different parameters $\lambda $ and $\mu$] \label{prop homotopie a parametres differents}
    Let $L$ be an $N$-reflexive polygonal chain, $F:= P_\lambda (L)$ and $F':= P_{\mu}(L)$ be two beams given respectively by $((a_i),(b_i))$ and $((a_i'),(b_i'))$, with respective parameters $\lambda$ and $\mu$ such that 
    \[
    K,K' < \min\biggl(d_R(L), \frac{d_O(L)}{2}\biggr)
    \]
    with $K:= \max\limits_{1 \leq j \leq N} \max (\lambda_j^a,\lambda_j^b)$ and $K':= \max\limits_{1 \leq j \leq N} \max (\mu_j^a,\mu_j^b)$, then $F\cong F'$.
\end{prop}

\begin{proof}
    Let us define the application $\gamma_{F,F'}$ as 
    \begin{align*}
        \gamma_{F,F'}: [0,1] &\longrightarrow \FaiscP \\
        t &\longmapsto (1-t)F + tF'
    \end{align*}
    where $(1-t)F + tF' = \Bigl( \bigl((1-t)a_i + ta_i' \bigr), \bigl((1-t)b_i+ tb_i'\bigr) \Bigr)$. \\  
    Notice that $\gamma_{F,F'}(t) = P_{(1-t)\lambda + t\mu}$, we then obtain that $\gamma_{F,F'}(t)$ is a beam for all $t$ in $[0,1]$ since we have by  \cref{corollaire faisceau P_l}
    \[
    \max\limits_{1 \leq j \leq N} \max \Bigl((1-t)\lambda_j^a + t\mu_j^a, (1-t)\lambda_j^b + t\mu_j^b \Bigr) \leq \max (K, K') < \min \biggl( d_R(L), \frac{d_O(L)}{2} \biggr).
    \]
    So, the beams $F$ and $F'$ are homotopic by the application $\gamma_{F,F'}$.
\end{proof}

\begin{defprop}[Subbeam]
\label{defprop subbeam}
    Let $F$ be an $N$-beam, we define the following primary beam
    \[
    F_\mu:= \bigl( P_{t_a}, P_{t_b} \bigr)
    \]
    where $t_a = \frac{1 - \mu}{2}$ et $t_b = \frac{1 + \mu}{2}$ with parameter $0 < \mu \leq 1$ (see  \cref{def:t-ligne brisee} on $t$-polygonal chain for more details). \\
    The primary beam $F_\mu$ is in $\Faisc$ for $\mu$ in $]0,1]$. \\
    We then say that $F_\mu$ is the subbeam of $F$ with parameter $\mu$.
\end{defprop}

\begin{proof}
We take $F_\mu$ with $\mu$ in $]0,1]$ and we write $F_\mu = \bigl((a_i^\mu),(b_i^\mu)\bigr)$. As $\mu \leq 1$, the mirror $S_k^\mu = [a_k^\mu b_k^\mu]$ is included in $S_k = [a_k b_k]$ for $k$ in $\llbracket 1,N \rrbracket$. Thus, the reflection condition for $F_\mu$ is verified. \\
\\
Moreover, for all element $x \in R_{j,\mu}^t$ where $R_{j,\mu}^t$ is the $j$-th ray of the $t$-polygonal chain of $F_\mu$, there exists $\nu$ in $[0,1]$ such that $x$ belongs to $R_j^\nu$, with $R_j^\nu$ the $j$-th ray of the $\nu$-polygonal chain of $F$. \\
So we have $R_{j,\nu}^t \, \cap \, S_k = \varnothing$ (with $0 \leq j \leq N$ and $1 \leq k \leq N+1$ such that $k \neq j,j+1$) by the non-obscuration condition of $F$. Thus, the non-obscuration condition for $F_\mu$ is verified. \\
We have the two conditions of a beam verified, and then $F_\mu$ is a beam.
\end{proof}

Let us notice that the beam $F$ can be written as $F_1$, the subbeam of $F$ with parameter $1$.

\begin{corollaire}[Homotopy of subbeams] \label{corollaire homotopie sous-faisceaux}
    Let $F$ be an $N$-beam and $F_\mu$ be a subbeam of $F$ with parameter $0 < \mu \leq 1$. We introduce the application $H^F_\mu$ defined as 
    \begin{align*}
        H^F_\mu: [0,1] &\longrightarrow \Faisc \\
        t &\longmapsto F_{1 + t(\mu - 1)}
    \end{align*}
    connecting $F = F_1$ to $F_\mu$. \\
    So, $F$ and $F_\mu$ are homotopic.
\end{corollaire}

\begin{theo} \label{thm invariance}
    Let $F, F'$ be in $\Faisc$ such that $\IFaisc(F) = \IFaisc(F')$, that is to say $\NFaisc(F) = \NFaisc(F')$ and $\CarFaisc(F) = \CarFaisc(F')$, then $F \cong F'$, or equivalently, $F$ and $F'$ are in the same connected component of $\Faisc$.
\end{theo}

\begin{proof}
    In order to show the theorem, we first focus on reflexive polygonal chains  produced by the beams $F$ et $F'$ with the application $M_R: \Faisc \rightarrow \LR$. That is why we write $L:= M_R(F)$ and $L':= M_R(F')$. As $\NR(L) = \NR(L')$ and $\Car(L) = \Car(L')$, we obtain by  \cref{prop_compo_LR} a path $\gamma_R: [0,1] \rightarrow \LR$ such that $\gamma_R (0) = L$ and $\gamma_R(1) = L'$.

    \bigskip

    Let us come back now to the general case of beams. To rely on the case of reflexive polygonal chains, we will define an application $P^\varepsilon: B \rightarrow \FaiscP$ with parameter $\varepsilon > 0$ with $B = \text{Im}(\gamma_R) $. \\
    We then define the application $P^\varepsilon: B \rightarrow \FaiscP$ as $P_{l_\varepsilon}$ (see definition \ref{def application P_l}) with $l_\varepsilon = \bigl((\varepsilon, \dots, \varepsilon), (\varepsilon, \dots, \varepsilon)\bigr)$. Explicitly, $P^\varepsilon$ is defined as
    \begin{align*}
        P^\varepsilon: B &\longrightarrow \FaiscP \\
        ((c_i), (\theta_j)) &\longmapsto ((a_i),(b_i))
    \end{align*}
    with 
    \[
    (a_i, b_i) = \begin{cases}
        (c_i,c_i) \text{ if } i = 0, N+1, \\
        \bigl( c_i + \varepsilon (\cos(\theta_i),\sin(\theta_i)), c_i - \varepsilon ( \cos(\theta_i),\sin(\theta_i)) \bigr) \text{ if } i \in \llbracket 1,N \rrbracket
    \end{cases}
    \]
    for $i$ in $\llbracket 0, N+1 \rrbracket$. \\
    We show there exists a parameter $\varepsilon>0$ small enough such that
    \[
    \text{Im}(P^\varepsilon) \subseteq \Faisc.
    \]
    We then check the two conditions for a primary beam to be a beam. In the following steps, we verify one after the other the reflection and non-obscuration conditions of a beam:
    \begin{enumerate}
        \item[$\circ$] (reflection) \label{etape 1 epsilon}  
        Recall that we have $\gamma_R: [0,1] \rightarrow \LR$, the path between $L = M_R(F)$ and $L' = M_R(F')$. We now take the function
        \begin{align*}
            \widetilde{d}_R = d_R \circ \gamma_R: [0,1] &\longrightarrow \mathbb{R}^+_* 
        \end{align*}
        that is continuous. As this function is continuous on a compact domain, the minimun of the function is reached and we write
        \[
        m_R:= \min\limits_{t \in [0,1]} \widetilde{d}_R(t) > 0.
        \]
        By taking $\varepsilon < m_R$, we have $P^\varepsilon(b)$ that verifies the reflection condtion of beams for all $b$ in $B$ by  \cref{prop faisceau P_l condition reflection}. 
        
        \item[$\circ$] (Non-obscuration) \label{etape 2 epsilon} 
        Let us now consider the function
        \begin{align*}
            \widetilde{d}_O = d_O \circ \gamma_R: [0,1] &\longrightarrow \mathbb{R}^+_* 
        \end{align*}
       and notice that $\widetilde{d}_O$ is continuous on a compact. Thus, the minimun of the function is reached and we write
        \[
            m_O:= \min\limits_{t \in [0,1]} \widetilde{d}_O(t) > 0.
        \]
        By taking $\varepsilon < \frac{m_O}{2}$, we have $P^\varepsilon(b)$ that verifies the non-obscuration condition of beams for all $b$ in $B$ by  \cref{prop faisceau P_l condition non obscuration}. 
    \end{enumerate}
\bigskip 

With the two steps above, we take 
\begin{equation} \label{eq:epsilon condition faisceau}
    \varepsilon < \min \Bigl( m_R , \frac{m_O}{2} \Bigr)
\end{equation}
and we then have $P^\varepsilon(\gamma_R(t))$ in $\Faisc$ for all $t$ in $[0,1]$. 
With condition \eqref{eq:epsilon condition faisceau}, we obtain the function  
\[
P_{F^\varepsilon}^{(F')^\varepsilon}:= P^\varepsilon \circ \gamma_R: [0,1] \longrightarrow \Faisc
\]
connecting $F^\varepsilon:= P^\varepsilon(F)$ to $(F')^\varepsilon:= P^\varepsilon(F')$. \\
Now we must show
\begin{gather*}
    F \cong F^\varepsilon \quad \text{ and } \quad F' \cong (F')^\varepsilon 
\end{gather*}
in order to get a beam homotopy between $F$ and $F'$. \\

We will show that $F$ is homotopic to $F^\varepsilon$ in two steps. In step \ref{homotopie etape 1}, we show that $F$ is homotopic to $F_\mu$, subbeam of $F$ with a good choice of $\mu$ for step \ref{homotopie etape 2} where we show that $F_\mu$ and $F^\varepsilon$ are homotopic. 
\begin{enumerate}
    \item \label{homotopie etape 1} 
    We write $\bigl((a_i^\mu), (b_i^\mu)\bigr)$ for the subbeam $F_\mu$ of $F$. It can be rewritten in the form of $P_l(L)$ (we recall that $L = M_R(F)$) with $l_\mu = \Bigl(\bigl((l_\mu)_j^a \bigr)_{1 \leq j \leq N} , \bigl( (l_\mu)_j^b \bigr)_{1 \leq j \leq N} \Bigr)$ which is given explicitly by 
    \[
    (l_\mu)_j^a = \Bigl| P_j^\frac{1}{2} - a_j^\mu \Bigr| \qquad (l_\mu)_j^b = \Bigl| P_j^\frac{1}{2} - b_j^\mu \Bigr|
    \]
    with $j$ in $\llbracket 1,N \rrbracket$ where $\bigl(P^\frac{1}{2}_i\bigr)$ centered polygonal chain of $F$ (see  \cref{def:ligne brisee centrale}). \\
    In the next step, we will take $\mu$ in $]0,1]$ low enough to get 
    \[
    K_\mu:= \max\limits_{1 \leq j \leq N} \max \bigl((l_\mu)_j^a,(l_\mu)_j^b \bigr) < \min\Bigl(d_R(L), \frac{d_O(L)}{2} \Bigr).
    \]
    We consider now the $H_\mu^F$ application from  \cref{corollaire homotopie sous-faisceaux} connecting $F$ to $F_\mu$.
    \item \label{homotopie etape 2}
    Thanks to the condition on $\mu$ considered in the previous step, we have 
    \[
    K_\mu < \min \bigl(d_R(L),\frac{d_O(L)}{2} \bigr) 
    \]
    and we also have
    \[
    \varepsilon < \min \bigl(d_R(L),\frac{d_O(L)}{2} \bigr),
    \]
    so we obtain by  \cref{prop homotopie a parametres differents} the path $\gamma_{F_\mu, F^\varepsilon}$ between $F_\mu$ and $F^\varepsilon$.
\end{enumerate}
Thus, we consider the concatenation of paths $P_F:= H^F_\mu \cdot \gamma_{F_\mu, F^\varepsilon}$ (see footnote \ref{footnote:concat} for the concatenation of paths) and we have $\gamma_L$ which connects $F$ to $F^\varepsilon$ and so $F \cong F^\varepsilon$. \\
The same reasoning can be done with $(F')^\varepsilon$ and $F'$ by considering $F'_\mu$ with an adapted $\mu$. Thus, we obtain in the same manner a path $P^{F'}$ connecting $(F')^\varepsilon$ to $F'$.

\bigskip

Finally, we have the path
\[
P_{F^\varepsilon}^{(F')^\varepsilon}:= (P_F \cdot P_{F^\varepsilon}^{(F')^\varepsilon}) \cdot P^{F'}    
\]
connecting the beam $F$ to the beam $F'$.
\end{proof}

\begin{corollaire}
    We have a characterization of the connected component of $\Faisc$, we have: 
    \[
    \pi_0 \bigl( \Faisc \bigr) \simeq \pi_0 \bigl( \LO \bigr) \times \{ -1, 1 \}^N
    \]
    with the application
    \begin{align*}
        \IFaisc: \Faisc &\longrightarrow \pi_0(\LO) \times \{ -1, 1 \}^N  \\
        F &\longmapsto \bigl(\NFaisc(F), \Car(F)\bigr)
    \end{align*}
\end{corollaire}

\begin{proof}
Let $F,F'$ be beams in $\Faisc$. If $F$ and $F'$ are in the same connected component, then we obtain $\IFaisc(F) = \IFaisc(F')$ by proposition \ref{prop:invariance}. \\
Reciprocally, if we have $\IFaisc(F) = \IFaisc(F')$ then $F$ and $F'$ are in the same connected component by theorem \ref{thm invariance}. \\
So, we find 
\[ 
\pi_0 \bigl(\Faisc \bigr) \simeq \pi_0 \bigl( \LO \bigr) \times \{ -1, 1 \}^N
\]
by noticing that $\IFaisc$ is a surjective application.
\end{proof}
We have shown that $\IFaisc$ is an exact topological invariant according to definition \ref{def:invariant} in the previous corollary.


==> inputs/beam_sym.tex <==
In  \cref{subsection:Faisc}, we have defined a beam $F$ as the data of two polygonal chains $\bigl( (a_i)_{0 \leq i \leq N+1},(b_i)_{0 \leq i \leq N+1} \bigr)$. If we consider now the beam $F'$ defined as $\bigl( (b_i), (a_i))$, we obtain two different beams which have nevertheless the same geometry when we represent them: the order does not have an influence on the interpretation of the beam. That is why we introduce in this subsection the space of symmetrical beams $\FaiscS$; the beams $F$ and $F'$ then produce the same symmetrical beam. 
Let us begin with
\begin{defi}[Signature] \label{def:signature faisceau}
    Let us define the \textit{signature} application as
    \begin{align*}
        \sign^F: \Faisc &\longrightarrow \{ -1, 1 \}^{N-1} \\
        F &\longmapsto \sign^F(F)
    \end{align*}
    with
    \[
    \sign^F(F)_k = \begin{cases}
        1 \text{ if } \CarFaisc(F)_k \text{ and } \CarFaisc(F)_{k+1} \text{ have the same sign,} \\
        -1 \text{ otherwise} \end{cases}
    \]
    for $1 \leq k \leq N-1$.
\end{defi}


We define a topological invariant $\IFaiscSym$ for $\FaiscS$ which is the conjunction of the two following invariants:
\begin{itemize}
    \item[$\circ$] the $\NFaiscSym$ application that comes from $\NFaisc$,
    \item[$\circ$] the $\signSym$ application that comes from $\sign^F$ (see \cref{def:signature faisceau}). We cannot indeed use the characteristic as an invariant since we have $\CarFaisc(F) = -\CarFaisc(F')$ but we have $\sign^F(F) = \sign^F(F')$.
\end{itemize}
We show that the invariant $\IFaiscSym$ is exact with  \cref{thm invariance symetrique}.

\begin{defi}[Symetrical beams]
    The discrete group $G = \mathbb{Z} / 2 \mathbb{Z}$ acts continuously on the space of beams $\Faisc$ by taking the action 
    \begin{align*}
        0 \cdot \bigl((a_i),(b_i)\bigr) &= \bigl((a_i),(b_i)\bigr) \\
        1 \cdot \bigl((a_i),(b_i)\bigr) &= \bigl((b_i),(a_i)\bigr)
    \end{align*}
    where $\mathbb{Z}/ 2\mathbb{Z}$ has two elements, $0$ (identity element) and $1$, with $1 + 1 = 0$ and where $\bigl((a_i),(b_i)\bigr)$ is a beam. \\
    We then define the space of \emph{symmetrical beams} $\FaiscS$ as 
    \[
    \FaiscS = G \backslash \Faisc .
    \]
\end{defi}

The orbit $O_F$ of an $N$-beam $F$ given by $\bigl((a_i),(b_i)\bigr)$ with the action of $G$ has two elements
\[
O_F = \{ F, \FI \}
\]
with $\FI = \bigl((b_i),(a_i)\bigr)$ that we call the inverse beam of $F$. The inverse beam is indeed different from $F$ since $a_1 \neq b_1$ (condition on the beams). We denote $\pi_S: \Faisc \rightarrow \FaiscS$ the quotient application and we will show in  \cref{lemme pi_S revetement} that $\pi_S$ is a covering.

\begin{prop} \label{prop faisceau symetrique caracterisation}
    Let $F$ be an $N$-beam given by $\bigl((a_i),(b_i)\bigr)$, then we have
    \[
    \NFaisc(F) = \NFaisc(\FI)
    \]
    where we recall that $\NFaisc$ is the nomenclature of beams. \\
    We also have
    \[
    \CarFaisc(F) = - \CarFaisc(\FI)
    \]
    with $\CarFaisc $ the characteristic of beams.
\end{prop}

\begin{proof}
    We directly have $\NFaisc(F) = \NFaisc(\FI)$ as $M(F) = M(\FI)$. \\
    Let us consider $L:= M_R(F)$ given by $\bigl((c_i),(\theta_j)\bigr)$ and $\LI:= M_R(\FI)$ given by $\bigl((c_i'),(\theta_j')\bigr)$. \\
    As $M(F) = M(\FI)$, we get $(c_i) = (c_i')$ and so
    \begin{align*}
        \Bigl( \Aplus \Bigr)_{1 \leq j \leq N} &= \Bigl( \Aplusp \Bigr)_{1 \leq j \leq N} \\
        \Bigl( \Aminus \Bigr)_{1 \leq j \leq N} &= \Bigl( \Aminusp \Bigr)_{1 \leq j \leq N}
    \end{align*}
    since orientation spaces of mirrors of $F$ and $\FI$ depend only on $(c_i)$ et $(c_i')$. \\
    The angles we obtain are
    \[ 
    \theta_j = A(a_j - b_j) = A(b_j - a_j) + \pi = \theta_j' + \pi
    \]
    we recall that $A: \mathbb{R}^2 \rightarrow \mathbb{R}/ 2\pi \mathbb{Z}$ is the angle function. \\
    Thus, if $\theta_j \in \Aplus$ then $\theta_j' \in \Aminusp$ and if $\theta_j \in \Aminus$ then $\theta_j' \in \Aplusp$. We then have
    \[
    \CarFaisc(F) = - \CarFaisc(\FI).
    \]
\end{proof}

We deduce from the previous proposition that we can define a nomenclature $\NFaiscSym$ for the symetrical beams that comes from $\NFaisc$ through the quotient application $\pi_S$. As we have $\NFaisc(F) = \NFaisc(\FI)$ for all beam $F$ , there exists an application $\NFaiscSym$ that verifies $\NFaisc = \NFaiscSym \circ \pi_S$. We represent the construction of this new nomenclature by the following commutative diagram  \\
\adjustbox{scale = 1.1, center}{
    \begin{tikzcd}
        \Faisc \arrow{d}{\pi_S} \arrow{r}{\NFaisc} & \pi_0(\LO) \\
        G \backslash \Faisc \arrow[dashed, swap]{ru}{\NFaiscSym}
    \end{tikzcd}
}
and we then have \[
\NFaiscSym(\mathcal{F}) = \NFaisc(F) = \NFaisc(\FI)
\]
where $\mathcal{F} \in \FaiscS$ is  the class of $F$ and $\FI$ in $\FaiscS$ that is $\pi_S(F) = \pi_S(\FI) = \mathcal{F}$. 
Likewise, we have $\sign^F(F) = \sign^F(\FI)$ as $\CarFaisc(F) = -\CarFaisc(\FI)$. So, we define the application $\sign^S$ for symmetrical beams that comes from $\sign^F: \Faisc \rightarrow \{ -1, 1 \}^{N-1}$ through the quotient application $\pi_S$. We then have
\[
\signSym(\mathcal{F}) = \sign^F(F) = \sign^F(\FI)
\]
where $\mathcal{F} \in \FaiscS$ and $\pi_S(F) = \pi_S(\FI) = \mathcal{F}$.

\begin{lemme} \label{lemme pi_S revetement}
    The $\pi_S: \Faisc \rightarrow \FaiscS$ application is a covering.
\end{lemme}

\begin{proof}
    Firstly, $\pi_S$ is surjective by definition. \\
    Moreover, $G$ acts freely on $\Faisc$ since $|G| = 2$ and every orbit of a beam $F$ has two elements  \[
    O_F = \{ F, \FI \}.
    \]
    So, $\pi_S: \Faisc \rightarrow G \backslash \Faisc$ is a covering because the discrete group $G$ acts freely on the space of beams, $\Faisc$, which is Haussdorff.
\end{proof}

We show in the next proposition that $\IFaiscSym:= (\NFaiscSym \times \signSym)$ is a topological invariant of $\FaiscS$.

\begin{prop}[Topological invariant: $\IFaiscSym$] \label{prop:invariant IS}
    Let $\gamma$ be a path connecting $\mathcal{F}$ to $\mathcal{F}'$ in $\FaiscS$, then
    \[
    \IFaiscSym(\mathcal{F}) = \IFaiscSym(\mathcal{F}')
    \]
    where we define $\IFaiscSym$ as 
    \begin{align*}
    \IFaiscSym: \FaiscS &\longrightarrow \pi_0(\LO) \times \{ -1, 1 \}^{N-1}  \\
    F &\longmapsto \bigl(\NFaiscSym(F), \signSym(F)\bigr).
    \end{align*}
\end{prop}

\begin{proof}
Let $F$ be a beam such that $\pi_S(F) = \mathcal{F}$. Recall that  $\pi_S: \Faisc \rightarrow \FaiscS$ is a covering by  \cref{lemme pi_S revetement},. \\
As $\gamma$ is a path starting from $\mathcal{F}$ such that $\pi_S(F) = \mathcal{F}$, there exists an only lift $\widetilde{\gamma}: [0,1] \rightarrow \Faisc$ of $\gamma$ (that means $\pi_S \circ \widetilde{\gamma} = \gamma$) such that $\widetilde{\gamma}(0) = F$ as $\pi_S$ is a covering. We represent the lifting property in the following commutative diagram.
\begin{center}
    \begin{tikzcd}
        {\{ 0 \}} \arrow{rr}{F} \arrow[hookrightarrow]{dd} && \Faisc \arrow{dd}{\pi_S} \\ \\
        {[0,1]} \arrow{rr}{\gamma} \arrow[dashed]{rruu}{\widetilde{\gamma}} && \FaiscS 
    \end{tikzcd}
\end{center}
We write $F':= \widetilde{\gamma}(1)$ and we have $\pi_S(F') = \mathcal{F}'$ from the commutativity of the diagram. We get that $F$ and $F'$ are in the same connected component as they are connected by $\widetilde{\gamma}$. \\
Thus, we have $\NFaisc(F) = \NFaisc(F')$ and $\sign(F) = \sign(F')$. We then obtain by definition of $\NFaiscSym$ and $\signSym$
\begin{gather*}
    \NFaiscSym(\mathcal{F}) = \NFaiscSym(\pi_S(F)) = \NFaisc(F) = \NFaisc(F') = \NFaiscSym(\pi_S(F')) = \NFaiscSym(\mathcal{F}'),  \\
    \signSym(\mathcal{F}) = \signSym(\pi_S(F)) = \sign^F(F) = \sign^F(F') = \signSym(\pi_S(F')) = \signSym(\mathcal{F}').
\end{gather*}
So we have $\IFaiscSym(\mathcal{F}) = \IFaiscSym(\mathcal{F}')$.
\end{proof}

\begin{theo} \label{thm invariance symetrique}
Let $\mathcal{F}$, $\mathcal{F}'$ be in $\FaiscS$ such that $\IFaiscSym(\mathcal{F}) = \IFaiscSym(\mathcal{F}')$, which means $\NFaiscSym(\mathcal{F}) = \NFaiscSym(\mathcal{F'})$ and $\signSym(\mathcal{F}) = \signSym(\mathcal{F}')$, then $\mathcal{F}$ and $\mathcal{F}'$ are in the same connected component of $\FaiscS$. 
\end{theo}

\begin{proof}
    In order to show the theorem, we take $F$ and $F'$ in $\Faisc$ such that $\pi_S(F) = \mathcal{F}$ and $\pi_S(F') = \mathcal{F}'$ where we choose $F$ such that $\CarFaisc(F)_1 = 1$ (we can substitute $F$ for $\FI$ if that is not the case as $\CarFaisc(F) = - \CarFaisc(\FI)$ by  \cref{prop faisceau symetrique caracterisation}). \\
    In the same way,we have without loss of generality $\Car(F')_1 = 1$. \\
    We have by definition of $\signSym$ 
    \begin{gather*}
        \signSym(\mathcal{F}) = \signSym(\pi_S(F)) = \sign(F), \\
        \signSym(\mathcal{F}') = \signSym(\pi_S(F)) = \sign(F').
    \end{gather*}
    so $\sign^F(F) = \sign^F(F')$.
    As we have $\CarFaisc(F)_1 = \CarFaisc(F')_1$ and $\sign(F) = \sign(F')$, we obtain 
    \[
    \CarFaisc(F) = \CarFaisc(F').
    \]
    As we notice that $\NFaiscSym(\mathcal{F}) = \NFaiscSym(\mathcal{F}')$, we have by definition of $\NFaiscSym$ 
    \[
    \NFaisc(F) = \NFaisc(F').
    \]
    So, there exists a beam homotopy $\gamma: [0,1] \rightarrow \Faisc$ connecting $F$ and $F'$ by theorem \ref{thm invariance}. Then, we consider the path 
    \[
    \Gamma:= \pi_S \circ \gamma: [0,1] \rightarrow \FaiscS
    \]
    between $\mathcal{F}$ and $\mathcal{F}'$.
\end{proof}


\begin{corollaire}
    We have a characterization of the connected components of $\FaiscS$:
    \[
    \pi_0 \bigl( \FaiscS \bigr) \simeq \pi_0 \bigl( \LO \bigr) \times \{ -1, 1 \}^{N-1}
    \]
    with the application
    \begin{align*}
        \IFaiscSym: \FaiscS &\longrightarrow \pi_0(\LO) \times \{ -1, 1 \}^{N-1}  \\
        F &\longmapsto \bigl(\NFaiscSym(F), \signSym(F)\bigr)
    \end{align*}
\end{corollaire}

\begin{proof}
Let $\mathcal{F}$, $\mathcal{F}'$ be in $\FaiscS$. If $\mathcal{F}$ and $\mathcal{F}'$ are in the same connected component, then we obtain $\IFaiscSym(\mathcal{F}) = \IFaiscSym(\mathcal{F}')$ by  \cref{prop:invariant IS}. \\
Reciprocally, if we have $\IFaiscSym(\mathcal{F}) = \IFaiscSym(\mathcal{F}')$ then $\mathcal{F}$ and $\mathcal{F}'$ are in the same connected component by   \cref{thm invariance symetrique}. \\
So, we find
\[ 
\pi_0 \bigl( \FaiscS \bigr) \simeq \pi_0 \bigl( \LO \bigr) \times \{ -1, 1 \}^{N-1}
\]
by noticing that $\IFaiscSym$ is a surjective application.
\end{proof}

We have shown that $\IFaiscSym$ s an exact topological invariant according to definition
\ref{def:invariant} in the previous corollary.


==> inputs/conclusion.tex <==
In this paper, we have extended the investigation of the connected components of the set of polygonal chains $\LO$, conducted in a previous work \cite{offaxis24}, to the connected components of the set of polygonal beams $\Faisc$.  Specifically, we demonstrate that an exact topological invariant can be obtained by incorporating the orientations of the mirrors alongside the one used to characterize the connected components of the set of polygonal chains. We finally deduce an exact topological invariant for the quotient space $\FaiscS$ obtained by the left action of the group $\mathbb{Z}/2\mathbb{Z}$ on $\Faisc$.
A future exploration would involve the algebraic constraints presented in \cite{onaxis24}. Indeed, let us introduce
%\begin{definition}[Magnifications] \label{def magnifications}
 the  \emph{magnifications} 
$(\Omega_k)_{1 \leq k \leq N-1}$ of $F$ by taking 
\begin{equation}
\Omega_k = \sign(F)_k \times \frac{|b_{k+1} - a_{k+1}|}{|b_k - a_k |}
\label{def magnifications}
\end{equation}
%\end{definition}
Let us consider  a polygonal chain $L:= (a_i)$, we obtain the signed distances, $d_k = (-1)^k|a_{k+1} - a_k|$ for $k=1,\dots ,N$.
Following \cite{onaxis24}, let us consider the set $E_{on}$, the real solutions of the two first-order equations called  \emph{focal} and \emph{Petzval's} ones in the case $N=3$. If  the discriminant coming from $L$ is positive or zero, we obtain two solutions in $(\Omega_1,\Omega_2)$ and an on-axis nomenclature encoding the sign of the magnifications and of the mirrors' curvatures \footnote{ For example the name $\texttt{PP101}$ means that the first and the second  magnifications are positive, the first mirror is convex, the second one is concave and the last one is convex.}.
Let us remark that these magnifications can serve, with the entrance pupil diameter (that is the data of $|a_1-b_1|$), to determine entirely the polygonal chain $(b_i)$ such that \eqref{def magnifications} would be satisfied. Besides from \cref{corollaire faisceau P_l} we know that there exists a subbeam $F_\mu$ with $0<\mu<1$ small enough such that $F_\mu$ is a beam (see \cref{defprop subbeam}).
% By solving the equations for the focal case of codimension 2 from \cite{offaxis24}, which gives us a set of admissible $E^3_{f,2}$ and get an \emph{on-axis} nomenclature if the discriminant coming from $L$ is positive or zero, we get two pairs of magnifications $(\Omega_1,\Omega_2)$ which can serve with the entrance pupil diameter (the data of $|a_1-b_1|$), to determine entirely the polygonal chain $(b_i)$ such that \cref{def magnifications} would be satisfied. Let $F$ the obtained beam, in order to take into account the obscuration constraint, it remains to search for $1>\mu>0$ such that the subbeam $F_\mu$ (see \cref{defprop subbeam} is a beam.
To illustrate numerically the paired \emph{on-off} axis topological invariants repartition for $N=3$ mirrors, solving the two first-order equations called \emph{focal} and \emph{Petzval} in \cite{onaxis24},
we  sample a million of polygonal chains  $(a_i) \in \text{LO}^3(\mathbb{R}^2)$ from a uniform law verifying $a_0 = (0,0)$, $a_1 = (0,1)$, $a_2$ in $[0,1] \times [-1,1]$ and also $a_3$ and $a_4$ in $[-1,1]^2$. 
We represent in  \Cref{fig:classification off-on axis} the optical systems distribution in the connected components of $E_{on}$ associated with each nomenclature of $\text{LO}^3(\mathbb{R}^2)$.
A future work to do is the mathematical study of the connected components for this paired model.

\begin{figure}[h!]
    \centering
    %\makebox[0.6\textwidth][c]{
    \includegraphics[trim={1cm 0 0 1.5cm},clip,width=.6\linewidth]{figures/off-on_axis.pdf}
   % }
    \caption{\textit{On-off} axis topological invariants repartition estimation for $N=3$ mirrors.}
    \label{fig:classification off-on axis}
\end{figure}


==> inputs/poly_chain.tex <==
This section presents the polygonal chains model derived in \cite{offaxis24}, which is the cornerstone of the beam light classification presented in the next sections.   
Here, we give the sketched ideas and refer the reader to \cite{offaxis24} for more details. 

Let us consider \(N+2\) points \((c_i)_{i = 0, \dots, N+1}\) in \(\mathbb{R}^2\)  to model the system: the half-line \((c_0, c_1]\) represents the direction of the source, the points \((c_j)_{j=1, \dots, N}\) correspond to the mirrors, and \(c_{N+1}\) represents the focal plane.  
Thus, we work within the space of \(N\)-polygonal chains \(\LB\), defined by:
\[
\LB:= \bigl(\mathbb{R}^2 \bigr)^{N+2}
\]
with the topology induced by \(\bigl(\mathbb{R}^2 \bigr)^{N+2}\).  
Let us first introduce the notion of a ray for a polygonal chain.

\begin{defi}[Ray for a polygonal chain] \label{def:rayon ligne brisee}
Let \(L\) be an \(N\)-polygonal chain given by \((c_i) \in \LB\). We denote the \(j\)-th ray as  
\[
R_j = 
\begin{cases}
    (c_0, c_1] & \text{if } j = 0, \\
    [c_j, c_{j+1}] & \text{if } j \in \llbracket 1, N \rrbracket
\end{cases}
\]
for \(j \in \llbracket 0, N \rrbracket\).
\end{defi}
On $\LB$, $R_0$ can be empty if $c_0=c_1$ and $R_j$ for $j\in \llbracket 1, N \rrbracket$ can be reduced to a point if $c_j=c_{j+1}$. Hence, we are going to add constraints so that these degenerate cases are not in the admissible set and such that there is not obscurating or grazing rays so that there is no loss of information.
To achieve this, we will define the required polynomials and explain their geometric significance, in order to define a space for admissible polygonal chains.
\begin{defi}[\cite{offaxis24}]
    Let us define
\[
\begin{cases} 
P = X_1Y_2 - X_1Y_3 + X_2Y_3-X_2Y_1 + X_3Y_1 - X_3Y_2 \\
R = (X_2 - X_1)(X_3-X_1) + (Y_2 - Y_1)(Y_3-Y_1)
\end{cases}
\]
where $ P, Q\in \mathbb{R}[X_1,X_2,X_3,Y_1,Y_2,Y_3]$.
Let  \[P_{(i,j,k)}, \, R_{(i,j,k)} \in \mathbb{Q}[X_0, \dots, X_{N+1}, Y_0, \dots, Y_{N+1}] \text{ defined by}\] 
\begin{align*}
     P_{(i,j,k)} &= P(X_i, X_j, X_k, Y_i, Y_j, Y_k) \textrm{ for } 
    0\leq i<j<k \leq N+1\land \min(j-i, k-j) = 1\\
    R_{(i, j, k)} &= R(X_i, X_j, X_k, Y_i, Y_j, Y_k)\text{ for }  0 \leq i,j,k \leq N+1 \text{ distinct and }|i-j| = 1
\end{align*}
\end{defi} 
\noindent
The defined polynomials have a geometric significance when specializing  
\[
(X_0, \dots, X_{N+1}, Y_0, \dots, Y_{N+1}) \text{ to } (x_0, \dots, x_{N+1}, y_0, \dots, y_{N+1}) 
\]
where \(c_j = (x_j, y_j)\).  In particular: 
\begin{itemize}
    \item[(i)]The polynomial \(P_{(i,j,k)}\) equals 0 if and only if the points \(c_i\), \(c_j\), and \(c_k\) are collinear.  
    \item[(ii)]The polynomial \(R_{(i,j,k)}\) is greater than or equal to 0 when \(P_{(i,j,k)} = 0\) if and only if \(c_k \in [c_i, c_j)\). Indeed, with the specialization, we can write \(R_{(i,j,k)} = (c_j - c_i) \cdot (c_k - c_i)\).
\end{itemize}

We introduce below the space studied for Off-Axis classification presented in \cite{offaxis24}. To this end, we define the obscuration clause $\varphi_{(i,j,k)}$ associated with the index $(i,j,k)$, which is satisfied if and only if $c_k$ is within the segment $[c_i, c_j]$ for $(i,j,k) \in \widetilde{S}_{\obsc}$, where  
\[
\widetilde{S}_{\obsc} = \Bigl\{ (i, i+1, k), \, 1 \leq i \leq N , \, 1 \leq k \leq N+1, \, k \not \in \{ i, i+1\} \Bigr\}.
\]  
Using the observation made above regarding the polynomials $P_{(i,j,k)}$ and $R_{(i,j,k)}$, we have  
\[
\varphi_{(i,j,k)} = (P_{\sigma(i,j,k)} = 0) 
\wedge (R_{(k,i,j)} \leq 0),
%\wedge (R_{(i,j,k)} \geq 0) \wedge (R_{(j,i,k)} \geq 0),
\]  
for $(i,j,k) \in \widetilde{S}_{\obsc}$, and with $\sigma$ being the permutation that orders $i$, $j$, and $k$ from smallest to largest.  
Furthermore, in the case where $i=0$, the obscuration clause is satisfied if and only if $c_k$ lies in the half-line $(c_0, c_1]$ for $k \in \llbracket 2; N+1\rrbracket$. We then introduce the set of indices $\widetilde{S}_{\obsc}'$ defined as  
\[
\widetilde{S}_{\obsc}' = \bigl\{ (0,1,k), \, k = \llbracket 2, N+1\rrbracket\bigr\}.
\]  
The obscuration clause for  $(i,j,k)\in \widetilde{S}_{\obsc}'$ is given by  
\[
\varphi_{(i,j,k)} = (P_{(i,j,k)} = 0) \wedge (R_{(j,i,k)} \geq 0).
\]
It is easily seen that $\widetilde{S}_{\obsc} \cap \widetilde{S}_{\obsc}' = \varnothing$ showing that the $\varphi_{i,j,k}$ are well defined.
\begin{defi}[Obscuration] \label{def:obscuration}
We define the obscuration clause $\obsc$ as 
\[
\obsc:= \bigvee\limits_{(i,j,k) \in S_{\obsc}} \varphi_{(i,j,k)}
\]
where $S_{\obsc}:= \widetilde{S}_{\obsc} \cup \widetilde{S}_{\obsc}'$.
\end{defi}

\begin{figure}[h!]
  \begin{subfigure}[b]{.32\textwidth}
    \centering
      \includegraphics[width=\textwidth]{figures/ligne_brisee_cas1.pdf}
      \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
       \includegraphics[width=\textwidth]{figures/ligne_brisee_cas2.pdf}
      \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
       \includegraphics[width=\textwidth]{figures/ligne_brisee_rasante.pdf}
      \caption{}
  \end{subfigure}
  \caption{Non admissible polygonal chains: (a) the mirror $c_4$ is obscuring the ray $R_1=[c_1,c_2]$, (b) the mirror $c_4$ is obscuring the light source $R_0=(c_0,c_1]$ and (c) the mirror $c_2$ is grazing since it belongs to $[c_1,c_3]$.}
  \label{fig:obscuration_grazing}
\end{figure}

In Figure \ref{fig:obscuration_grazing}, we depict two broken $4$-lines that are obscured. The one shown in (a) satisfies $\varphi_{(1,2,4)}$ because $c_4$ belongs to the segment $[c_1, c_2]$. The second (depicted in (b)) is obscured because we observe that $c_4$ lies on the light source: $c_4$ belongs to $(c_0, c_1]$. Thus, $\varphi_{(0,1,4)}$ is satisfied for the polygonal chain $c = (c_0, \dots, c_5)$, and therefore, the polygonal chain is obscured.

\begin{remark} \label{rem:obscuration}
    The obscuration clause $\obsc$ for the polygonal chain $L = (c_i) \in \LB$ can be equivalently rewritten using the concept of a ray:  
\[
\obsc = \bigvee_{0 \leq j \leq N} \bigvee_{\substack{1 \leq k \leq N+1 \\ k \neq j,j+1}} \bigl( R_j \cap c_k \neq \varnothing \bigr).
\]
\end{remark}

We now introduce a new clause defining grazing, i.e., the cases where the polygonal chain has three consecutive points aligned in order.  
To this end, we introduce the set \( S_{\ras} = \{ (m-1,m,m+1) \, , \, 1 \leq m \leq N \} \) and define the grazing clause for indices \((i,j,k)\) in \(S_{\ras}\):  
\[
\psi_{(i,j,k)} = \bigl( P_{(i,j,k)} = 0 \wedge R_{(j,i,k)} \leq 0 \bigr).
\]

\begin{defi}[Grazing] \label{def:rasance}
We define the grazing clause $\ras$ as 
\[
\ras:= \bigvee\limits_{(i,j,k) \in S_{\ras}} \psi_{(i,j,k)}.
\]
\end{defi}
\begin{remark}\label{re:grazing}
    The grazing clause $\ras$ holds true if a degenerate ray exists. Indeed, if $R_0=\emptyset$ then $\psi_{(0,1,2)}=\texttt{true}$ and if there exists $j\in \llbracket 2,N\rrbracket$ such that $R_j=\{c_j\}$ then $\psi_{j-1,j,j+1}=\texttt{true}$.
\end{remark}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.6\textwidth]{figures/ligne_brisee_rasante.pdf}
%     \caption{Grazing polygonal chain.}
%     \label{fig:rasance}
% \end{figure} 

In \Cref{fig:obscuration_grazing}-(c), the points $c_1$, $c_2$, and $c_3$ are aligned, so $P_{(1,2,3)}(c) = 0$ and $R_{(2,1,3)} < 0$, where $c$ is the polygonal chain represented in the figure. Thus, the grazing clause $\psi_{(1,2,3)}$ is satisfied for this polygonal chain so that the system is grazing.


\begin{defi}[Space $\LO$] \label{def:LO}
We first define the joint clause of obscuration and grazing as $\ObscRas = \obsc \vee \ras$. The non-admissible polygonal chains subspace is defined as \( E_{\ObscRas} = \bigl\{ c \in \LB\,: \, \ObscRas(c) \bigr\} \). We then define the space of $N$-polygonal chains under obscuration and grazing constraints as:  
\[
\LO:= \LB \backslash E_{\ObscRas}.
\]
\end{defi}

\begin{defi} [Exact Invariant: Off-Axis Nomenclature] \label{def nomenclature}  
We introduce the nomenclature, denoted as  
\begin{align*}  
\N: \LO \rightarrow \pi_0 \bigl(\LO \bigr),  
\end{align*}  
where $\pi_0(\LO)$ is the set of connected components of $\LO$. We define $\N$ by taking $\N(L) = \N(L')$ if and only if $L$ and $L'$ are in the same connected component of $\LO$, for $L$ and $L'$ in $\LO$.  
\end{defi}



The nomenclature is therefore by definition an exact invariant in the sense of \cref{def:invariant}: it is even the canonical exact invariant since it directly uses the connected components of the space.

We have an explicit characterization of the nomenclature called the GOFFA (geometrical off-axis) nomenclature. This nomenclature, denoted by $\NGOFFA$, is introduced in \cite{offaxis24}, and the following theorem shows that it is an exact invariant in specific cases.


\begin{theo}[\cite{offaxis24}] \label{theoreme_nomenclature}
    The nomenclature given by $\NGOFFA: \LO \rightarrow B$ is an invariant of the space $\LO$. It is an exact invariant for $N= 3,4$ mirrors.
\end{theo}


Let us explain in more detail how the nomenclature $\NGOFFA$ assigns a name to each polygonal chain. The name of a system is given recursively on its mirrors. For a polygonal chain $L = (c_i)_{0 \leq i \leq N+1} \in \LO$, we process the mirrors step by step in the order $j = 1, \dots, N$.

At step $j$, we consider the segment $[c_j, c_{j+1}]$. If this segment does not intersect any of the previous segments $[c_k, c_{k+1}]$ for $1 \leq k < j$ or the light source $(c_0, c_1]$, then we assign the letter $V$ to the $j$-th mirror. Otherwise, we assign the letter $X$, and we also indicate as subscripts the segments and/or the half-line (for the light source) that are intersected by the segment $[c_j, c_{j+1}]$. 

Furthermore, we add the letter $A$ or $C$ ($A$ for \emph{anticlockwise} and $C$ for \emph{clockwise}) as a subscript to indicate the direction of rotation of the ray at the $j$-th mirror. This is explicitly given by the sign of $(c_{j+1}-c_j) \wedge (c_{j-1}- c_j)$, where $\wedge$ is the cross product given by  
\[
\begin{pmatrix}x \\ y \end{pmatrix} \wedge \begin{pmatrix}x' \\ y' \end{pmatrix} = xy' - x'y'.
\]
For $N=3$, these 3 invariants are sufficient. For $N=4$, an additional invariant that considers the set of points enclosed by a subset of the polygonal chain is necessary.
Thus, we observe that, up to symmetry with respect to the first mirror, all names begin with $V_A$.  
The space $\text{LO}^3(\mathbb{R}^2)$ has 32 connected components and 16 up to symmetry while the space $\text{LO}^4(\mathbb{R}^2)$ has 288 connected components and 144 up to symmetry.


==> inputs/reflexive_chain.tex <==
In this section, we introduce the space $\LR$ of reflexive polygonal chains, which provides a more accurate representation of optical systems than the space $\LO$ defined in the previous subsection. 
From now, when there is no possibility of confusion, we denote $(c_i)$ as the sequence $(c_i)_{i\in I}$ when the index set $I \subset \mathbb{N}$ has been clearly specified beforehand.
 Mirrors are no longer just points; each now has an angle representing its direction. This introduces a new condition which is named \emph{reflection}. After defining this new space, we introduce two topological invariants:  
\begin{itemize}  
    \item[$\circ$] the nomenclature $\NR$, inspired by $\N$ defined in \cref{def nomenclature},  
    \item[$\circ$] the characteristic $\Car$ (see definition \ref{def:caracteristique}).  
\end{itemize}  
Finally, we show that the joint invariant $\IR = (\NR \times \Car)$ is an exact invariant  \cref{prop_compo_LR}.


\begin{defi}[Reflexive polygonal chain] \label{def lignes brisees reflexives}
An $N$-reflexive polygonal chain is defined as a polygonal chain $(c_i)_{0 \leq i \leq N+1} \in \LO$ together with angles $(\theta_j)_{1 \leq j \leq N} \in (\mathbb{R}/2\pi \mathbb{Z})^N$ (associated with each mirror) that satisfy the following condition:  
\[
\forall \, \, 1 \leq j \leq N, \, \sgn \bigl((c_{j+1} - c_j) \cdot n(\theta_j) \bigr)=\sgn \bigl((c_{j-1} - c_j) \cdot n(\theta_j) \bigr) \neq 0
\]
where $n(\theta)$ is the unit normal of the line defined by the angle $\theta$, and $\sgn$ is the sign function defined as follows:  

\begin{align*}
    \sgn: \mathbb{R} & \longrightarrow \{ -1, 0, 1 \} \\
    x & \longmapsto \begin{cases}
        1 \text{ if } x>0, \\
        -1 \text{ if } x<0, \\
        0 \text{ if } x=0.
    \end{cases}
\end{align*}

The space of reflexive polygonal chains is denoted as $\LR$.

\end{defi}

Geometrically, the condition for being a \emph{reflexive polygonal chain} means that $c_{j-1}$ and $c_{j+1}$ lie in the same half-plane bounded by the line passing through $c_j$ and  of angle $\theta_j$.


\begin{figure}[h!]
    \centering
    \begin{subfigure}[b]{.45\textwidth}
    \includegraphics[width=\textwidth]{figures/angle_admissible_cas1.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{.45\textwidth}
    \includegraphics[width=\textwidth]{figures/angle_admissible_cas2.pdf}
    \end{subfigure}
    \caption{Admissible angles for reflexive polygonal chains.}
    \label{fig:reflexion}
\end{figure}

In \Cref{fig:reflexion}, we illustrate the points $c_{j-1}$, $c_j$, and $c_{j+1}$ for two different polygonal chains in $\LO$. The gray region in each case corresponds to the admissible area for the angle $\theta_j$ to satisfy the reflection condition at this point: the angle, represented as an element of the circle $\mathbb{R}/2\pi\mathbb{Z}$, must then belong to the red displayed circles. We observe that as the angle between the half-lines $[c_j c_{j-1})$ and $[c_j c_{j+1})$, denoted by $\phi$ in the figure, increases toward $\pi$, the space of admissible angles decreases. The limiting case where $\phi$ equals $\pi$ corresponds to the grazing case illustrated in  \Cref{fig:obscuration_grazing}-(c) for polygonal chains.


\begin{defi}[Application \(M_O\)] \label{def application M_O}
    An \(N\)-reflexive polygonal chain \(L\), given by \((c_i)\) and \((\theta_j)\), induces a polygonal chain in \(\LO\) via the application:
    \[
    \begin{aligned}
         M_O:\LR &\longrightarrow \LO \\
        L&\longmapsto (c_i)_{0 \leq i \leq N+1}.
    \end{aligned}
    \]
    where we recall that \(L = \bigl( (c_i), (\theta_j) \bigr)\).
\end{defi}

\begin{defi}[Ray of a Reflexive Polygonal Chain] \label{def:rayon_LR}
    Let \(L\) be an \(N\)-reflexive polygonal chain given by \(((c_i), (\theta_j))\). 
    The \(j\)-th ray is defined as the ray of \(M_O(L) \in \LO\) as defined in  \cref{def:rayon_LR}.
\end{defi}

\begin{defi}[Nomenclature \(\NR\)] \label{def:nomenclature reflexive}
    We define the nomenclature \(\NR\) for reflexive polygonal chains as the application:
    \[
    \begin{aligned}
        \NR: \LR &\longrightarrow \pi_0(\LO) \\
        L &\longmapsto \N((c_i)),
    \end{aligned}
    \]
    where \(L = \bigl( (c_i), (\theta_j) \bigr)\). 
    Thus, we have \(\NR = \N \circ M_O\).
\end{defi}

\begin{prop}[Topological Invariant: \(\NR\)] \label{prop invariance ligne brisee reflexive nomenclature}
    Let \(L\) and \(L'\) be in \(\LR\) such that there exists a continuous path \(\gammaR\) connecting \(L\) to \(L'\), then \(\NR(L) = \NR(L')\).
\end{prop}


\begin{proof}
    Consider the composition \(M_O \circ \gammaR: [0,1] \rightarrow \LO\) which connects \(L_*:= M_O(L)\) to \(L_*':= M_O(L')\). We have:
    \[
    \N(L_*) = \N(L_*')
    \]
    since \(\N\) is a topological invariant by the definition of the nomenclature in \(\LO\) (see  \cref{def nomenclature}). Thus, we find:
    \[
    \NR(L) = \N(L_*) = \N(L_*') = \NR(L')
    \]
    by the definition of the nomenclature in \(\LR\) (see  \cref{def:nomenclature reflexive}).
\end{proof}
It is also possible to define the reflection condition of reflexive polygonal chains using the angle function \( A: \mathbb{R}^2 \rightarrow \mathbb{R}/2\pi \mathbb{Z} \) which, for a non-zero vector \(x\), returns the angle \(\theta\) such that \( x = r \bigl( \cos( \theta), \sin(\theta) \bigr) \) for a unique \( r > 0 \); we will discuss this perspective further below.

\begin{defi}[Orientations of Mirrors] \label{def orientation miroirs}
    Let \( L \in \LO \) be an \( N \)-polygonal chain given by \( (c_i) \). We define the orientation spaces of the mirrors with the spaces \( (\Aplus \) (positive orientation) and \( (\Aminus \) (negative orientation) for the \( j \)-th mirror with \( 1 \leq j \leq N \) as:
    \begin{align*}
        \Aplus &= \bigl( A(c_j - c_{j-1}) + (-1)^j \, ]0, \pi [ \bigr) \cap \bigl( A(c_j - c_{j+1}) + (-1)^j \, ]0, \pi [ \bigr) \\
        \Aminus &= \bigl( A(c_j -c_{j-1}) + (-1)^{j+1} \, ]0, \pi [ \bigr) \cap \bigl( A(c_j - c_{j+1}) + (-1)^{j+1} \, ]0, \pi [ \bigr)
    \end{align*}
\end{defi}

Note that this also defines the orientation spaces of the mirrors for a reflexive polygonal chain \( L_R \in \LR \) by taking \( L = M_O(L_R) \).

\begin{remark} \label{convexite orientation miroirs}
    In  \cref{def orientation miroirs}, we defined the spaces \( \Aplus \) and \( \Aminus \) for a polygonal chain \( L \in \LO \) and \( 1 \leq j \leq N \). Note that these two spaces are connected. Let us take elements \( a, \, b \in \Aplus \). Suppose first that \( b - a \) has a representative in \( [0, \pi[ \) which we denote by \( R(b - a) \). We then consider the path 
    \begin{align*}
        \gamma_{a,b}: [0,1] &\longrightarrow \mathbb{R}/2 \pi \mathbb{Z} \\ 
        t &\longmapsto a + tR(b - a)
    \end{align*}
    which is a path from \( a \) to \( b \) that satisfies
    \[
    \forall \, t \in [0,1], \, \gamma_{a,b}(t) \in \Aplus
    \]
    by definition of \( \Aplus \). Therefore, the points \( a \) and \( b \) are connected by the linear path \( \gamma_{a,b} \). \\
    Similarly, when \( a - b \) has a representative in \( [0, \pi[ \), we obtain the path \( \gamma_{b,a} \) by the previous reasoning. We then take the inverse path of \( \gamma_{b,a} \) to connect \( a \) to \( b \), that is, \( \gamma_{b,a} \circ \text{\normalfont{Inv}} \), where \( \text{\normalfont{Inv}}: [0,1] \rightarrow [0,1] \) is defined by \( \text{\normalfont{Inv}}(t) = 1 - t \). \\
    This same reasoning can be adapted for the space \( \Aminus \).
\end{remark}

We can then define reflexive polygonal chains from  \cref{def lignes brisees reflexives} equivalently using the mirror orientations. Indeed, given a polygonal chain $L = (c_i) \in \LO$ and angles $(\theta_j)\in(\mathbb{R}\backslash 2\pi\mathbb{Z})^N$, the data $((c_i),(\theta_j))$ satisfies the reflexive polygonal chain condition if and only if
\[
\forall \, 1 \leq j \leq N, \, \theta_j \in \Aplus \text{ or } \theta_j \in \Aminus.
\]

We will introduce a new topological invariant, in the sense of  \cref{def:invariant}, for the space $\LR$ called the \textit{characteristic}, which takes into account the positive or negative orientation of the mirrors (see  \cref{def orientation miroirs}).

\begin{defi}[Characteristic] \label{def:caracteristique}
Let $L$ be a $N$-reflexive polygonal chain given by the polygonal chain $(c_i)$ and angles $(\theta_j)$. The \textit{characteristic} of $L$, denoted $\Car(L)$, is an element of $\{ -1 ,1 \}^N$ and is defined as follows:
\[
\Car(L)_j = \begin{cases}
    1 \text{ if } \theta_j \in \Aplus, \\
    -1 \text{ if } \theta_j \in \Aminus,
\end{cases}
\]
with $j \in \llbracket 1, N \rrbracket$.
\end{defi}

We represent the characteristic in  \Cref{fig: orientation} by depicting two reflexive polygonal chains $L$ and $L'$ at a mirror. The first, denoted $L$, is given by $(c_0,c_1,c_2) \in \LO$ and the angle $\theta \in \mathbb{R}/ 2\pi\mathbb{Z}$ as shown in the figure by the blue arrow. We then have $\Car(L)_1 = -1$ since $\theta$ is in the blue area representing $(\mathcal{A}_L^-)_1$. Similarly, the second reflexive polygonal chain $L'$ is also given by $(c_0,c_1,c_2)$ and the angle $\theta'$ represented on the figure by the red arrow. We then find $\Car(L)_1 = 1$ since $\theta'$ is in the red area representing $(\mathcal{A}_{L'}^+)_1$. Note that we have the following relations:
\begin{gather*}
    (\mathcal{A}_{L'}^-)_1 = (\mathcal{A}_L^-)_1, \quad
    (\mathcal{A}_{L'}^+)_1 = (\mathcal{A}_L^+)_1,
\end{gather*}
since $L$ and $L'$ share the same underlying polygonal chain, i.e., $M_O(L) = M_O(L')$.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/caracteristique.pdf}
    \caption{Caracteristic for two polygonal chains $L$ and $L'$}
    \label{fig: orientation}
\end{figure}


\begin{prop}[Topological Invariant: $\Car$] \label{prop invariance ligne brisee reflexive car}
    Let $L$ and $L'$ be in $\LR$ such that there exists a continuous path $\gammaR: [0,1] \rightarrow \LR$ connecting $L$ to $L'$, then $ \Car(L) = \Car(L')$.
\end{prop}

\begin{proof}
    Suppose, by contradiction, that there exists a path $\gammaR: [0,1] \rightarrow \LR$ such that $\gammaR(0) = L$ and $\gammaR(1) = L'$ and some $k \in \llbracket 1, N \rrbracket$ such that 
    \[
    \Car(L)_k \neq \Car(L')_k.
    \]
    Without loss of generality, assume that $\Car(L)_k = 1$ and $\Car(L')_k = -1$. \\
    Let $\gammaR(t) = \bigl((c_i^t)_{0 \leq i \leq N+1}, (\theta_i^t)_{1 \leq i \leq N} \bigr)$ where $(c_i^t) \in \LO$ and $(\theta_i^t) \in (\mathbb{R} / 2\pi \mathbb{Z})^N$. \\
    Specifically, we are interested in the evolution of the angle $\theta^t_k$ over time because it is at index $k$ that the characteristic of $L$ and $L'$ differs. To study this, we introduce the function 
    \begin{align*}
        \gamma_k^\theta: [0,1] &\longrightarrow \mathbb{R} / 2\pi \mathbb{Z} \\
        t &\longmapsto \theta_k^t - A(c_k^t - c_{k-1}^t)
    \end{align*}
    and it follows from the hypothesis that $R(\gamma_k^\theta(0)) \in (-1)^k \, ]0, \pi[$ and $R(\gamma_k^\theta(1)) \in (-1)^{k+1} ]0, \pi[$ (with $R$ being the bijection from $\mathbb{R} / 2\pi \mathbb{Z}$ to $ ]-\pi , \pi ]$), since $\theta_k^0 \in \mathcal{A}_k^+$ and $\theta_k^1 \in \mathcal{A}_k^-$. \\
    Notice that the function $\gamma_k^\theta$ is continuous and the space $(\mathbb{R}/2\pi \mathbb{Z}) \backslash \{0 ,\pi \}$ decomposes into two connected components, $ ]-\pi, 0[$ and $ ]0, \pi[$. Thus, since $R(\gamma_k^\theta(0)) \in (-1)^k]0, \pi[$ and $R(\gamma_k^\theta(0)) \in (-1)^{k+1}]0, \pi[$, there exists some $t \in [0,1]$ such that $R(\gamma_k^\theta(t)) = 0$ or $R(\gamma_k^\theta(t)) = \pi$. \\
    We then obtain $\sgn\bigl((c_{k-1}^t - c_k^t) \cdot n(\theta_k^t)\bigr) = 0$ because the line $(c_{k-1}^t, c_k^t)$ coincides with the line spanned by $\theta_k^t$ at $c_k$. This leads to a contradiction since the condition for a reflexive polygonal chain is violated.
\end{proof}

The following results will be useful to prove  \cref{prop_compo_LR}.

\begin{defi}[Bisectors]
    Let $m_2$ be the covering map\footnote{A covering map is a map $p: \widetilde{X} \rightarrow X$ between topological spaces such that for each point $x \in X$, there exists a neighborhood $U_x$ of $x$ and a discrete space $D_x$ satisfying \[
    p^{-1}(U_x) = \bigsqcup\limits_{d \in D_x} V_d \quad  \text{ and } \quad p|_{V_d}: V_d \rightarrow X \text{ is a homeomorphism for each } d \in D_x.
    \]
     For more details, refer to Chapter 1 of \cite{Hatcher02}.} of $\mathbb{S}^1 =  \mathbb{R}/ 2\pi \mathbb{Z}$ given by
    \begin{align*}
            m_2: \mathbb{R}/ 2\pi \mathbb{Z} &\longrightarrow \mathbb{R}/ 2\pi \mathbb{Z} \\
            x &\longmapsto 2x.
    \end{align*}
    Let $L \in \LO$ be given by $(c_i)$. We define the \textit{bisectors} (for $1 \leq j \leq N$) of $L$ as the elements in the fiber of $\psi(L)_j$ under $m_2$, where
    \begin{align*}
        \psi: \LO &\longrightarrow (\mathbb{R} /2\pi \mathbb{Z})^N \\
        L=(c_i)_{0 \leq i \leq N+1} &\longmapsto \bigl( A(c_{j-1} - c_j) + A(c_j - c_{j+1}) \bigr)_{1 \leq j \leq N}
    \end{align*}
    and we denote by $(B_L)_j$ the fiber of $\psi(L)_j$ under $m_2$.
\end{defi}

The following definition is used to prove  \cref{prop bissectrices} on the explicit characterization of the bisectors.

\begin{defi}[Circle Distance]
We define a distance $d_{\mathbb{S}^1}$ on the circle as
\begin{align*}
    d_{\mathbb{S}^1}: \mathbb{R}/2\pi \mathbb{Z} &\longrightarrow \mathbb{R}^+ \\
    (x,y) &\longmapsto \min \Bigl\{ \bigl| (R(x) + 2\pi k) - (R(y) + 2 \pi k')\bigr| \,: \, k, k' \in \mathbb{Z}  \Bigr\}
\end{align*}
where $R$ is the representation map from $\mathbb{R}/2\pi \mathbb{Z}$ to $[0, 2 \pi[$.
\end{defi}

\begin{prop} \label{prop bissectrices}
    Let $L \in \LO$, the set  $(B_L)_j$ of $L$ consists of two elements, denoted 
    \[
    (B_L)_j = \bigl\{ (B_L^+)_j, (B_L^-)_j \bigr\}
    \]
    where $(B_L^+)_j \in \Aplus$ and $(B_L^-)_j \in \Aminus$.
\end{prop}

\begin{proof}
Notice that the fiber of $\psi(L)_j$ under $m_2$ consists of two elements, denoted $x$ and $y$, with $x = y + \pi$. Therefore, it is not possible to have both $x$ and $y$ in $\Aplus$ or both in $\Aminus$. Indeed, for two points $z, z'$ in $\Aplus$ or $\Aminus$, we have $d_{\mathbb{S}^1}(z, z') < \pi$ by definition, while $d_{\mathbb{S}^1}(x, y) = \pi$. 

Moreover, we can geometrically interpret $(B_L)_j$ by noting that it consists of the bisectors of the half-lines $[c_jc_{j-1})$ and $[c_j c^+_j)$ on one side, and $[c_j, c_{j+1})$ and $[ c_j, c^-_j )$ on the other side, where $c^+_j = c_j + (c_j - c_{j+1})$ and $c_j^- = c_j + (c_j - c_{j-1})$. We illustrate this in  \Cref{fig: bissectrices off axis} for $j = 1$. In this figure, we represent the orientations of the first mirror (at $c_1$) by the red part for $(\mathcal{A}_L^+)_1$ and the blue for $(\mathcal{A}_L^-)_1$. The red and blue arrows in the figure represent the bisection lines $(B_L^+)_1$ and $(B_L^-)_1$ of the reflexive polygonal chain, respectively. \\
Thanks to this description, it is clear that $c_{j-1}$ and $c_{j+1}$ lie in the same half-plane defined by either of the bisection lines. \\
Thus, by possibly switching the notation, we obtain
\begin{align*}
    x \in \Aplus & \text{ and } y \in \Aminus.
\end{align*}


\end{proof}
\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{figures/bissectrice.pdf}
    \caption{Illustration of $(B_L^+)_1$ and $(B_L^-)_1$}
    \label{fig: bissectrices off axis}
\end{figure}
    
Before presenting the following lemma, which we will use to prove  \cref{prop_compo_LR}, we extend the definition of characteristic to work with arbitrary angles. Let $\phi = (\varphi_j) \in (\mathbb{R}/ 2\pi \mathbb{Z})^N$ associated with an $N$-reflexive polygonal chain $L$, by defining
\[
\Car_L(\phi)_j = \begin{cases}
    1 \text{ if } \varphi_j \in \Aplus, \\
    -1 \text{ if } \varphi_j \in \Aminus, \\
    0 \text{ otherwise.}
\end{cases}
\]

\begin{lemme} \label{homotopie angles}
Let $L$ be an $N$-reflexive polygonal chain given by $(c_i) \in \LO$ and $(\theta_j) \in (\mathbb{R}/ 2\pi \mathbb{Z})^N$, and let $\phi = (\varphi_j) \in (\mathbb{R}/ 2\pi \mathbb{Z})^N$ such that $\Car_L(\phi) = \Car(L)$. Then $L$ and the $N$-reflexive polygonal chain $L'$, given by $(c_i)$ and $(\varphi_j)$, are in the same connected component of $\LR$.
\end{lemme}

\begin{proof}
    Using the notation from the lemma, we construct a path $\gamma: [0,1] \rightarrow \LR$ such that $\gamma(0) = L$ and $\gamma(1) = L'$ to show that $L$ and $L'$ are in the same connected component of $\LR$. \\
    Using  \cref{convexite orientation miroirs}, we define $\gamma$ as
    \begin{align*}
    \gamma: [0,1] &\longrightarrow \LR \\
    t &\longmapsto \bigl( (c_i), (\gamma_{\theta_j, \varphi_j}(t)) \bigr)    
    \end{align*}
    which is well-defined since
    \[
    \gamma_{\theta_j, \varphi_j}(t) \in \begin{cases}
        \Aplus & \text{if } \theta_j \in \Aplus, \\
        \Aminus & \text{if } \theta_j \in \Aminus.
    \end{cases}
    \]
    for every $j$ in $\llbracket 1, N \rrbracket$ and $t\in [0,1]$ by   \cref{convexite orientation miroirs}.
\end{proof}

To show that by considering both topological invariants $\NR$ and $\Car$ together, we obtain an exact invariant $\IR:= (\NR \times \Car)$ of the space $\LR$, we prove the other implication of   \cref{def:invariant}.

\begin{prop} \label{prop_compo_LR}
Let $L$, $L'$ be elements of $\LR$ such that $\NR(L) = \NR(L')$ and $\Car(L) = \Car(L')$. Then there exists a path $\gamma_R: [0,1] \rightarrow \LR$ such that $\gamma_R(0) = L$ and $\gamma_R(1) = L'$. Therefore, $L$ and $L'$ are in the same connected component of the space $\LR$.
\end{prop}

\begin{proof}
    To prove the proposition, we first focus on $M_O(L)$ and $M_O(L')$, where we define $M_O: \LR \rightarrow \LO$ in \cref{def application M_O}. Since $\NR(L) = \NR(L')$, $M_O(L)$ and $M_O(L')$ are in the same connected component, so there exists a path 
    \begin{align*}
        P: [0,1] &\longrightarrow \LR
    \end{align*} 
    connecting $M_O(L)$ and $M_O(L')$.
    We now want to find a lift $\widetilde{P}_R: [0,1] \rightarrow \LR$ of $P$ through the map $M_O: \LR \rightarrow \LO$, which sends a reflexive polygonal chain $((c_i),(\theta_j))$ to $(c_i)$, such that $\widetilde{P}_R(0) = L_*$ and $\widetilde{P}_R(1) = L_*'$, where we define the reflexive polygonal chains $L_*$ and $L_*'$ in steps \ref{etape 1} and \ref{etape 2} below. These reflexive polygonal chains satisfy the following properties:
    \begin{itemize}
        \item[$\circ$] There exists a path $\gamma_L: [0,1] \rightarrow \LR$ (constructed in step \ref{etape 1}) such that $\gamma_L(0) = L$ and $\gamma_L(1) = L_*$,
        \item[$\circ$] There exists a path $\gamma_{L'}: [0,1] \rightarrow \LR$ (constructed in step \ref{etape 3}) such that $\gamma_{L'}(0) = L_*'$ and $\gamma_{L'}(1) = L'$.   
    \end{itemize}
    The lifting property of $\widetilde{P}_R$ is illustrated by the following commutative diagram:
    \begin{center}
        \begin{tikzcd} 
        {\{ 0 \}} \arrow[bend left = 15]{rrrr}{L_*} \arrow[hookrightarrow]{ddr} & {\{ 1 \}} \arrow[hookrightarrow]{dd} \arrow{rrr}{L_*'} &&& \LR \arrow{dd}{M_O} \\ \\ 
        & {[0,1]} \arrow{rrr}{P} \arrow[dashed]{rrruu}{\widetilde{P}_R} &&& \LO 
        \end{tikzcd}
    \end{center}

    To construct $\widetilde{P}_R$ (which is done in step \ref{etape 2}), we first observe that the first component of $\widetilde{P}_R$ is determined. Indeed, since $M_O \circ \widetilde{P}_R = P$ by commutativity of the diagram, we can write $\widetilde{P}_R (t) = (P(t), (\varphi^t_j))$ where the angles $\phi^t = (\varphi^t_j) \in (\mathbb{R}/ 2\pi \mathbb{Z})^N$ need to be determined. Additionally, we have
    \begin{gather*}
        M_O(L) = P(0) = M_O(L_*), \\
        M_O(L') = P(1) = M_O(L_*').
    \end{gather*} 
    We proceed in three steps, which we detail below:
    \begin{enumerate}
        \item \label{etape 1} Starting from $L$ given by $(c_i) \in \LO$ and the angles $(\theta_j) \in (\mathbb{R}/ 2\pi \mathbb{Z})^N$, we want to construct a path from $L$ to $L_*$ given by $(c_i)$ and the angles $B^0 = (B^0_j)$ defined as
        \[
        B^0_j = \begin{cases}
            (B_L^+)_j \text{ if } \theta_j \in \Aplus, \\
            (B_L^-)_j \text{ if } \theta_j \in \Aminus,
        \end{cases}
        \]
        with the notation from  \cref{prop bissectrices}. \\
        Since $\Car_L(B^0) = \Car(L)$, there exists a path $\gamma_L: [0,1] \rightarrow \LR$ connecting $L$ to $L_*$ by  \cref{homotopie angles}.
        We now note that
        \[
        \Car(L) = \Car(L_*).
        \]
        \item \label{etape 2} Now, starting from $L_*$, we will construct a lift $\widetilde{g}_j$ of the path $g_j$ (for each $j$ in $\llbracket 1, N \rrbracket$), defined as
        \begin{align*}
            g_j: [0,1] &\longrightarrow \mathbb{R} / 2\pi \mathbb{Z} \\
            t &\longmapsto A\bigl( P_{j-1}(t) - P_j(t) \bigr) + A \bigl( P_j(t) - P_{j+1}(t) \bigr),
        \end{align*}
        by $m_2: \mathbb{R}/  2\pi \mathbb{Z} \rightarrow \mathbb{R}/  2\pi \mathbb{Z}$ such that $\widetilde{g}_j(0) = B^0_j$, as illustrated by the following commutative diagram:
        \[
        \adjustbox{scale=1.1,center}{
        \begin{tikzcd} 
            {\{ 0 \}} \arrow{r}{B^0_j} \arrow[hookrightarrow]{d} & \mathbb{R}/  2\pi \mathbb{Z} \arrow{d}{m_2} \\
            {[0,1]} \arrow{r}{g_j} \arrow[dashed]{ur}{\widetilde{g}_j} & \mathbb{R}/  2\pi \mathbb{Z}
        \end{tikzcd}
        }
        \]
        Since $m_2$ is a covering map, there exists a unique lift $\widetilde{g}_j$ of the path $g_j$ through $m_2$ such that $\widetilde{g}_j(0) = B^0_j$. Thus, denoting $\widetilde{g} = (\widetilde{g}_j)_{1 \leq j \leq N}$, we consider the continuous path
        \begin{align*}
            \widetilde{P}_R: [0,1] &\longrightarrow \LR \\
            t &\longmapsto (P(t), \widetilde{g}(t)),
        \end{align*}
        which is well-defined by  \cref{prop bissectrices}.
        This path satisfies $\widetilde{P}_R(0) = L_*$, and we define the endpoint of the path as $L_*':= \widetilde{P}_R(1)$. We now note that
        \[
        \Car(L_*) = \Car\bigl(L_*' \bigr)
        \]
        by  \cref{prop invariance ligne brisee reflexive car}.
        \item \label{etape 3} This step consists of reversing step \ref{etape 1}: we want to find a path $\gamma_{L'}$ from $L_*'$ to $L'$, with $L'$ given by $(c'_i) \in \LO$ and the angles $(\theta'_j) \in (\mathbb{R}/ 2 \pi \mathbb{Z})^N$. Note that $L_*' = \widetilde{P}_R (1) = (P(1), \widetilde{g}(1)) = ((c'_i), \widetilde{g}(1))$ because $P(1) = (c_i')$. Using the equalities
        \[
        \Car(L') = \Car(L) = \Car(L_*) = \Car \bigl( L_*' \bigr)
        \]
        by steps \ref{etape 1} and \ref{etape 2} and the hypothesis of the theorem, we obtain $\Car_{L'} (B^1) = \Car(L')$ where $B^1 = \widetilde{g}(1)$. Thus, there exists a path $\gamma_{L'}$ connecting $L_*'$ to $L'$ by  \cref{homotopie angles}.
    \end{enumerate}
    We must concatenate the paths given in steps \ref{etape 1}, \ref{etape 2}, and \ref{etape 3} in order to construct the path $\gamma_R$ that connects $L$ to $L'$. We then define
    \[
    \gamma_R:= (\gamma_L \cdot \widetilde{P}_R) \cdot \gamma_{L'}
    \]
    where $\cdot$ denotes the path concatenation operator\footnote{Let two paths $\alpha, \beta: [0,1] \rightarrow X$ such that $\alpha(1) = \beta(0)$ with $X$ a topological space. We denote by $\alpha \cdot \beta$ the path
    \[
    t \mapsto \begin{cases}
        \alpha(2t) \text{ if } t \in [0,\frac{1}{2}], \\
        \beta(2t-1) \text{ if } t \in [\frac{1}{2},1].
    \end{cases}
    \]
    \label{footnote:concat}}

\end{proof}

\begin{corollaire}[Exact Invariant of $\LR$] \label{corollaire:LR invariant}
    We have a characterization of the connected components of the space of reflexive polygonal chains $\LR$ by the nomenclature $\NR$ and the characteristic $\Car$: we have
    \[
    \pi_0 \bigl(\LR \bigr) \simeq \pi_0 \bigl( \LO \bigr) \times \{ -1, 1 \}^N
    \]
    via the map 
    \begin{align*}
        \IR: \LR &\longrightarrow \pi_0 \bigl( \LO \bigr) \times \{ -1, 1 \}^N  \\
        L &\longmapsto \bigl( \NR(L), \Car(L) \bigr).
    \end{align*}
\end{corollaire}

\begin{proof}
Let $L$ and $L'$ be reflexive polygonal chains in $\LR$. If $L$ and $L'$ are in the same connected component, then we have
\begin{gather*}
    \NR(L) = \NR(L') \, \text{ and } \,\Car(L) = \Car(L')
\end{gather*}
since $\NR$ and $\Car$ are topological invariants by  \cref{prop invariance ligne brisee reflexive nomenclature} and \cref{prop invariance ligne brisee reflexive car}. \\
Conversely, if we have
\begin{gather*}
    \NR(L) = \NR(L') \, \text{ and } \,\Car(L) = \Car(L')
\end{gather*}
then $L$ and $L'$ are in the same connected component by  \cref{prop_compo_LR}. \\
This shows that $\IR = (\NR \times \Car)$ is an exact topological invariant in the sense of  \cref{def:invariant}.

\medskip

We then have $\pi_0 \bigl(\LR \bigr) \cong \text{Im}(\IR)$. To show the result, we now prove that the map $\IR$ is surjective. Let $X_{\text{N}} \in \pi_0 \bigl( \LO \bigr)$ and $S \in \{ -1,1 \}^N$, then let $L \in \LO$ such that $\NR(L) = X_{\text{N}}$ and choose the angles $(\theta_j)$ with
\[
\theta_j = \begin{cases}
            (B_L^+)_j \text{ if } S_j = 1 \\
            (B_L^-)_j \text{ if } S_j = -1.
        \end{cases}
\]
for $j \in \llbracket 1, N \rrbracket$.
We then construct the reflexive polygonal chain $\widetilde{L} = \bigl(L, (\theta_j)\bigr)$ which satisfies $\IR \bigl(\widetilde{L} \bigr) = \bigl(X_{\text{N}}, S \bigr)$.

\end{proof}



==> inputs/tab1.tex <==
\begin{tabular}[t]{lll}
\toprule
off axis & on axis & percentage \\
\midrule
\multirow[t]{10}{*}{$V_AV_AV_A$} & $PP100$ & 0.00260 \\
 & $PP110$ & 0.17164 \\
 & $PP001$ & 0.22098 \\
 & $PP011$ & 1.06140 \\
 & $NP101$ & 1.48040 \\
 & $PN011$ & 1.59244 \\
 & $PP010$ & 2.06004 \\
 & $NP110$ & 2.56876 \\
 & $PN101$ & 2.68080 \\
 & $PP101$ & 3.08562 \\
\cline{1-3}
\multirow[t]{10}{*}{$V_AV_AV_C$} & $PP100$ & 0.00274 \\
 & $PP110$ & 0.20482 \\
 & $PP001$ & 0.32044 \\
 & $NP101$ & 2.13842 \\
 & $PP011$ & 2.22250 \\
 & $PP010$ & 2.37674 \\
 & $NP110$ & 2.85058 \\
 & $PN011$ & 3.04826 \\
 & $PN101$ & 3.76042 \\
 & $PP101$ & 4.51308 \\
\cline{1-3}
\multirow[t]{10}{*}{$V_AV_AX^3_{A,0}$} & $PP100$ & 0.00038 \\
 & $PP110$ & 0.01354 \\
 & $PP010$ & 1.15456 \\
 & $PP001$ & 1.43272 \\
 & $NP110$ & 1.88376 \\
 & $PN101$ & 2.68562 \\
 & $NP101$ & 5.05856 \\
 & $PP101$ & 5.14926 \\
 & $PP011$ & 5.28806 \\
 & $PN011$ & 5.86042 \\
\cline{1-3}
\multirow[t]{10}{*}{$V_AV_AX^3_{A,1}$} & $PP100$ & 0.00038 \\
 & $PP110$ & 0.06998 \\
 & $PN101$ & 0.86392 \\
 & $PP001$ & 1.44314 \\
 & $PP010$ & 1.97502 \\
 & $NP110$ & 2.93536 \\
 & $PN011$ & 3.66552 \\
 & $PP011$ & 3.90886 \\
 & $PP101$ & 4.61270 \\
 & $NP101$ & 5.73696 \\
\cline{1-3}
\end{tabular}


==> inputs/tab2.tex <==
\begin{tabular}[t]{lll}
\toprule
off axis & on axis & percentage \\
\midrule
\multirow[t]{10}{*}
{$V_AV_AX^3_{C,0}$} & $PP100$ & 0.00002 \\
 & $PP110$ & 0.00826 \\
 & $PP001$ & 0.05846 \\
 & $PN011$ & 0.08866 \\
 & $PN101$ & 0.10844 \\
 & $PP011$ & 0.17626 \\
 & $PP010$ & 0.37062 \\
 & $NP101$ & 0.46342 \\
 & $NP110$ & 0.48320 \\
 & $PP101$ & 0.49726 \\
\cline{1-3}
\multirow[t]{10}{*}{$V_AV_CV_A$} & $PP100$ & 0.00424 \\
 & $PP110$ & 0.23364 \\
 & $PP001$ & 0.44068 \\
 & $NP101$ & 3.70350 \\
 & $PP010$ & 3.88204 \\
 & $NP110$ & 5.09046 \\
 & $PP011$ & 6.74570 \\
 & $PN011$ & 9.17340 \\
 & $PP101$ & 10.46450 \\
 & $PN101$ & 10.56036 \\
\cline{1-3}
\multirow[t]{10}{*}{$V_AV_CV_C$} & $PP100$ & 0.00410 \\
 & $PP110$ & 0.20380 \\
 & $PP001$ & 1.92158 \\
 & $PP010$ & 4.50162 \\
 & $NP110$ & 6.60692 \\
 & $NP101$ & 8.56852 \\
 & $PP011$ & 11.06704 \\
 & $PN101$ & 12.25892 \\
 & $PP101$ & 14.00522 \\
 & $PN011$ & 14.22052 \\
\cline{1-3}
\multirow[t]{10}{*}{$V_AV_CX^3_{A,0}$} & $PP100$ & 0.00010 \\
 & $PP110$ & 0.00336 \\
 & $PP010$ & 0.09560 \\
 & $NP110$ & 0.13946 \\
 & $PP001$ & 0.14056 \\
 & $PN101$ & 0.23256 \\
 & $PP101$ & 0.30720 \\
 & $PP011$ & 0.33554 \\
 & $NP101$ & 0.34364 \\
 & $PN011$ & 0.43674 \\
\cline{1-3}
\end{tabular}

==> inputs/tab3.tex <==
\begin{tabular}[t]{lll}
\multirow[t]{10}{*}{$V_AV_CX^3_{C,01}$} & $PP100$ & 0.00006 \\
 & $PP110$ & 0.00732 \\
 & $PN101$ & 0.39440 \\
 & $PP010$ & 0.75932 \\
 & $PP001$ & 1.05396 \\
 & $NP110$ & 1.35798 \\
 & $PP101$ & 2.07740 \\
 & $PN011$ & 2.23626 \\
 & $PP011$ & 2.27822 \\
 & $NP101$ & 3.19984 \\
\cline{1-3}
\multirow[t]{10}{*}{$V_AV_CX^3_{C,0}$} & $PP100$ & 0.00002 \\
 & $PP110$ & 0.00046 \\
 & $PP010$ & 0.08940 \\
 & $NP110$ & 0.11258 \\
 & $PP001$ & 0.48176 \\
 & $NP101$ & 1.86814 \\
 & $PN101$ & 2.29616 \\
 & $PP101$ & 3.27064 \\
 & $PP011$ & 3.59512 \\
 & $PN011$ & 4.05172 \\
\cline{1-3}
\multirow[t]{10}{*}{$V_AV_CX^3_{C,1}$} & $PP100$ & 0.00046 \\
 & $PP110$ & 0.06306 \\
 & $PP001$ & 0.97836 \\
 & $PN101$ & 1.42180 \\
 & $PP010$ & 1.52992 \\
 & $NP110$ & 1.98042 \\
 & $PP011$ & 4.56756 \\
 & $PN011$ & 4.61432 \\
 & $NP101$ & 5.17294 \\
 & $PP101$ & 5.26872 \\
\cline{1-3}
\multirow[t]{10}{*}{$V_AX^2_{A,0}V_A$} & $PP100$ & 0.00134 \\
 & $PP110$ & 0.02052 \\
 & $PP001$ & 0.76638 \\
 & $PP010$ & 1.27074 \\
 & $NP110$ & 2.12702 \\
 & $NP101$ & 3.81922 \\
 & $PP011$ & 7.94372 \\
 & $PP101$ & 8.55678 \\
 & $PN101$ & 8.69252 \\
 & $PN011$ & 10.38472 \\
\cline{1-3}
\end{tabular}

==> inputs/tab4.tex <==
\begin{tabular}[t]{lll}
\multirow[t]{10}{*}{$V_AX^2_{A,0}V_C$} & $PP100$ & 0.00092 \\
 & $PP001$ & 0.00962 \\
 & $PP110$ & 0.01916 \\
 & $NP101$ & 0.34994 \\
 & $PP010$ & 0.92186 \\
 & $PP011$ & 1.44656 \\
 & $NP110$ & 1.51460 \\
 & $PP101$ & 2.37956 \\
 & $PN011$ & 2.64686 \\
 & $PN101$ & 3.81152 \\
\cline{1-3}
\multirow[t]{10}{*}{$V_AX^2_{A,0}X^3_{A,01}$} & $PP100$ & 0.00004 \\
 & $PP110$ & 0.00354 \\
 & $PP010$ & 0.30490 \\
 & $NP110$ & 0.40212 \\
 & $PP001$ & 0.58820 \\
 & $PN101$ & 0.95064 \\
 & $NP101$ & 2.62854 \\
 & $PP101$ & 2.72558 \\
 & $PP011$ & 2.93534 \\
 & $PN011$ & 3.17706 \\
\cline{1-3}
\multirow[t]{10}{*}{$V_AX^2_{A,0}X^3_{A,0}$} & $PP100$ & 0.00002 \\
 & $PP001$ & 0.00024 \\
 & $PP110$ & 0.00222 \\
 & $NP101$ & 0.09696 \\
 & $PP010$ & 0.10578 \\
 & $NP110$ & 0.14256 \\
 & $PP011$ & 0.35230 \\
 & $PN011$ & 0.43776 \\
 & $PP101$ & 0.46012 \\
 & $PN101$ & 0.48336 \\
\cline{1-3}
\multirow[t]{10}{*}{$V_AX^2_{A,0}X^3_{C,0}$} & $PP100$ & 0.00024 \\
 & $PP110$ & 0.00550 \\
 & $PP001$ & 0.18136 \\
 & $PP010$ & 0.29878 \\
 & $NP110$ & 0.36554 \\
 & $NP101$ & 1.08908 \\
 & $PN101$ & 3.08048 \\
 & $PP011$ & 3.22256 \\
 & $PP101$ & 3.36884 \\
 & $PN011$ & 3.80402 \\
\cline{1-3}
\end{tabular}

==> inputs/tab_topo.tex <==
\tiny

\begin{tabular}{@{} p{.45\linewidth} | p{.45\linewidth} @{}}   
\vtop{\centering % Aligne en haut et centre horizontalement
\input{inputs/tab1}}&
 \vtop{\centering 
\input{inputs/tab2}}\\
\vtop{\centering 
\input{inputs/tab3}}&
 \vtop{\centering 
\input{inputs/tab4}}
\end{tabular}


% \begin{tabular}{@{} p{.45\linewidth} | p{.45\linewidth} @{}}   
% \vtop{\centering % Aligne en haut et centre horizontalement
% \input{inputs/tab3.tex}}
% &\vtop{\centering % Aligne en haut et centre horizontalement
% \input{inputs/tab4.tex}}
% \end{tabular}
\normalsize
